Meerkat: A framework for Dynamic Graph Algorithms on GPUs

Graph algorithms are challenging to implement due to their varying topology and irregular access patterns. Real-world graphs are dynamic in nature and routinely undergo edge and vertex additions, as well as, deletions. Typical examples of dynamic graphs are social networks, collaboration networks, and road networks. Applying static algorithms repeatedly on dynamic graphs is inefficient. Unfortunately, we know little about how to efficiently process dynamic graphs on massively parallel architectures such as GPUs. Existing approaches to represent and process dynamic graphs are either not general or inefficient. In this work, we propose a library-based framework for dynamic graph algorithms that proposes a GPU-tailored graph representation and exploits the warp-cooperative execution model. The library, named Meerkat, builds upon a recently proposed dynamic graph representation on GPUs. This representation exploits a hashtable-based mechanism to store a vertex's neighborhood. Meerkat also enables fast iteration through a group of vertices, such as the whole set of vertices or the neighbors of a vertex. Based on the efficient iterative patterns encoded in Meerkat, we implement dynamic versions of the popular graph algorithms such as breadth-first search, single-source shortest paths, triangle counting, weakly connected components, and PageRank. Compared to the state-of-the-art dynamic graph analytics framework Hornet, Meerkat is $12.6\times$, $12.94\times$, and $6.1\times$ faster, for query, insert, and delete operations, respectively. Using a variety of real-world graphs, we observe that Meerkat significantly improves the efficiency of the underlying dynamic graph algorithm. Meerkat performs $1.17\times$ for BFS, $1.32\times$ for SSSP, $1.74\times$ for PageRank, and $6.08\times$ for WCC, better than Hornet on average.

==> algorithms/allocationcheme.tex <==
\REM{
\begin{algorithm}[H]
  \DontPrintSemicolon
  \SetKwFunction{SlabHashCtor}{SlabHashCtor}
  \SetKwFunction{SlabGraphCtor}{SlabGraphCtor}
  \SetKwProg{Fn}{function}{:}{}

  \SetKwData{V}{v}
  \SetKwData{VertexN}{vertex\_n}
  \SetKwData{SlabSize}{SLAB\_SIZE}
  \SetKwData{BucketsN}{buckets\_n}
  \SetKwData{HeadSlabs}{head\_slabs}
  \SetKwData{HeadSlabsVec}{head\_slabs\_vec}
  \SetKwData{VertexAdjacencies}{vertex\_adjacencies}
  \SetKwData{Index}{i}
  \SetKwData{BucketCount}{bucket\_count}
  \SetKwData{BucketOffset}{bucket\_offset}

  \SetKw{True}{true}
  \SetKw{False}{false}
  \SetKw{In}{in}

  \SetKwFunction{CudaMalloc}{cudaMalloc}
  \SetKwFunction{ExclusiveScan}{exclusive\_scan}

  \Fn() {\SlabHashCtor{\BucketsN, \HeadSlabsVec}} { \label{new:slabhash-ctor-signature}
    $\cdots$ \;
    \For{\Index \In \texttt{0}\ \dots\ \BucketsN}{ \label{new:loop-start}
      \HeadSlabs\texttt{[\Index]} $\leftarrow$ \HeadSlabsVec\texttt{[\Index]} \label{new:assign-pointer-offset} \;
    } \label{new:loop-end}
    $\cdots$ \;
  }

  \Fn() {\SlabGraphCtor{\VertexN}} {
    $\cdots$ \;
    \tcc{Compute bucket count for each vertex in bucket\_count; offsets for head slabs in bucket\_offset}
    \BucketOffset $\leftarrow$ \ExclusiveScan{\BucketCount\texttt{[0$\dots$\VertexN]}} \label{new:compute-offset} \;
    \BucketsN $\leftarrow$ \BucketOffset\texttt{[\VertexN\ -\ 1]} + \BucketCount\texttt{[\VertexN\ -\ 1]} \label{new:compute-buckets} \;
    \tcc{Allocate all head slabs as single block}
    \HeadSlabs $\leftarrow$ \CudaMalloc{\texttt{\&}\HeadSlabs\texttt{[0]}, \SlabSize $\times$ \BucketsN} \label{new:allocate-slabs} \;

    \For{\Index \In \texttt{0}\ \dots\ \VertexN}{ \label{new:ctor-loop-start}
      \VertexAdjacencies[\Index] = \SlabHashCtor{\BucketCount\texttt{[\Index]},\ \texttt{\&}\HeadSlabs\texttt{[\BucketOffset[\Index]]}} \label{new:pass-offsets} \;
    } \label{new:ctor-loop-end}
    $\cdots$ \;
  }
  \caption{Allocation Scheme: Inside \SG}
  \label{algorithm:allocation-inside-slabgraph}
\end{algorithm}
}

==> algorithms/bfs-deletehelper.tex <==
    \begin{algorithm}[t]
	    \small
%    \algrestore{BFS}
	
    \setcounter{AlgoLine}{0}
    \SetKw{True}{true}
  \SetKw{False}{false}
	\SetKwFunction{FHelper}{DeleteHelper}
 %   \SetKwProg{Fn}{Function}{:}{}
 \SetKwProg{Fn}{Function}{\{}{\}}

	    \Fn{\FHelper{\texttt{Graph} G, \texttt{Graph} BDAG, \texttt{int } Dist d[$n$], \texttt{EdgeSet} E'},\texttt{VertexSet} $Q_1$, \texttt{VertexSet} $Q_2$)}{
	    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	    \SetKwInOut{Requires}{Requires}
	    \SetKwInput{InParallel}{in parallel}
        \SetKwRepeat{Do}{do}{while}
%	    \Input{$G$ : Input graph}
%	    \Input{$BDAG$ : DAG for base graph}
%	    \Input{$d$ : Distance array for each vertex from source}
%	    \Input{$src$ : Source Vertex}
%	    \Input{$E'$ : Set of Edges in batch update}
%	    \Output{$d$ : Updates the distance array}
	    \BlankLine
	    %\texttt{VertexSet} $Q_1$ = $\phi$ \textcolor{brown}{ UK:Till end of for loop, it  happens in the host code} \\
	   % \texttt{VertexSet} $Q_2$ = $\phi$  \textcolor{brown}{ UK:Q1,Q2 passed as argument to DeleteHelper}\\
	   % \For{((u, v) $\in$ E')} {\label{ricky:BFS2:initpushbegin}
	    %    \uIf{(BDAG.parent[v] == \{u\})} {
	     %       $Q_1$.insertVertex(v) \\
	      %      d[v] = INF
	       % }
	    %}\label{ricky:BFS2:initpushend}
	    %\BlankLine
	    
	    %\Do{($changed$)} {\label{ricky:BFS2:deleteloopbegin}
	  %%\textcolor{brown}{UK:only device code, host code commented}\\
	\texttt{Vertex\_Dictionary} *vert\_adjs[] = G.get\_vertex\_adjacencies() \;
	%\todo{changed = \False}\\
    \If{(thread\_id() - lane\_id() $\textless$ vertex\_n)}{
        \texttt{bool} to\_process = (thread\_id() $\textless$ vertex\_n)\; %\ ? \True : \False \;
        \texttt{int} work\_queue = 0 \;
        %\While{((work\_queue = ballot\_sync(0$\times$FFFFFFFF, to\_process)) $\neq$ 0)} {
          \texttt{int} current\_lane = ffs(work\_queue) - 1 \;
          \texttt{int} index = (thread\_id() - lane\_id() + current\_lane) \;
          \texttt{Vertex} u = $Q_1$[index] \REM{ \textcolor{brown}{UK:Ricky, This should be u=$Q_1$[index]?, in the source code CurrentVertex=Modified1[ThreadID - LaneID + Lane]}} \;
          \tcc{Process source vertex}
          \texttt{SlabIterator} iter = vert\_adjs[u].begin() \;
          \texttt{SlabIterator} last =  vert\_adjs[u].end() \;
          \tcc{Iterate over adjacent vertices}
          \While{(iter $\neq$ last)} { 
          \texttt{Vertex}  v = *(iter.get\_pointer(lane\_id())) \;
            \If{(is\_valid\_vertex(v))} { 
              \uIf{(BDAG.parent[v] == \{u\} and d[v] $\neq$ INF)} {
	                    d[v] = INF \\
                        $Q_2$.insertVertex(v) \\
                        BDAG.deleteEdge(u, v) \\
                        changed = \True
                    }
            }
            ++iter \;
          }
          \tcc{Post-processing}
          \lIf{(index == thread\_id())} {
            to\_process = \False
          }
        } 
    }
	        
	        
%	        \For{ (u $\in$ $Q_1$ \textbf{in parallel})} { 
%	            \For{(v $\in$ adj(u, BDAG))} {
%	                \uIf{(BDAG.parent[v] == \{u\} and d[v] $\neq$ INF)} {
%	                    d[v] = INF \\
%                        $Q_2$.insertVertex(v) \\
%                        BDAG.deleteEdge(u, v) \\
%                        changed = \texttt{true}
%                    }
%	                \BlankLine
%                    \textbf{endif}
%               }
%	            \BlankLine
%	        }
	        %%\textcolor{brown}{UK:device code ends here}\\
	        %$Q_1$.clear(), $Q_1$.copy($Q_2$), $Q_2$.clear()\textcolor{brown}{UK:This is host code}\\
	   % }\label{ricky:BFS2:deleteloopend}
	%}
	\BlankLine
%	\textbf{End Function}
	    	
	\caption{DeleteHelper for Decremental BFS}
		\label{ricky:BFS1}

%    \algstore{BFS}
    \end{algorithm}


==> algorithms/bfs.tex <==
\begin{algorithm}[t]
	    \small

	
	\DontPrintSemicolon
	%\caption{\textsc\textsf{Dynamic BFS}}
	\tcc{Initialise BDAG for base graph $G$}
	\SetKwFunction{FMain}{InitBDAG}
 %   \SetKwProg{Fn}{Function}{:}{}
 \texttt{int} changed = 1\\
 \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}
    	\Fn{\FMain{\texttt{Graph} G, \texttt{Graph} BDAG}}{

	$BDAG = $ empty graph \label{ricky:BFS2:initBDAGbegin}\\
	\For{$((u, v) \in G.E)\ \textbf{in parallel}$} {
	    \If{$(d[v] == d[u] + 1)$}{
            BDAG.insertEdge(u, v)
        }
	    %\textbf{end if}
        }\label{ricky:BFS2:initBDAGend}
	   %\textbf{end for}
    	}

\REM{	\tcc{BFS routine modifies $d$ to hold the correct distance of each vertex from $src$}
	\SetKw{True}{true}
  \SetKw{False}{false}
	\SetKwFunction{FMain}{BFS}
    %\SetKwProg{Fn}{Function}{:}{}
    \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}

	\Fn{\FMain{\texttt{Graph} G, \texttt{int} Dist d[0$\dots$vertex\_n \todo{vertexn-1? if yes, check others}], \texttt{Vertex} src)}}{
	    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	    \SetKwInOut{Requires}{Requires}
	    \SetKwInput{InParallel}{in parallel}
        \SetKwRepeat{Do}{do}{while}
%	    \Input{$G$ : Input graph}
%	    \Input{$d$ : Distance array for each vertex from source}
%	    \Input{$src$ : Source Vertex}
%	    \Output{$d$ : Updates the distance array}
	    \BlankLine
	    
	    \Do{(changed)} {
	        \texttt{bool} changed = false \\
	        \For{$((u, v) \in G.E)$ \textbf{in parallel}} {
	            \uIf{(d[u] + 1 $<$ d[v])}{
	                \BlankLine
                    d[v] = d[u] + 1 \\
                    changed = \texttt{true}
                }
	            \BlankLine
                \textbf{endif}
	        }
	        \BlankLine
	    }
	    \BlankLine
	    
	}
	\textbf{End Function}
	}
\BlankLine		%\tcc{Incremental BFS}

	\SetKwFunction{FInsert}{IncrementalBFS}
    %\SetKwProg{Pr}{Function}{:}{}
    \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}

	   % \Fn{\FInsert{\texttt{Graph} G, \texttt{Vertex} src,\texttt{int} dist d[0$\dots$vertex\_n], \texttt{EdgeSet} E'}}{
%	    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%	    \Input{$G$ : Base graph}
%	    \Input{$src$ : Source Vertex}
%	    \Input{$d$ : Distance array for each vertex from source}
%	    \Input{$E'$ : Set of Edges in batch update}
	    %\BlankLine
	    
	    %\For{(u, v) $\in$ E') \textbf{in parallel}} {\label{ricky:BFS3:insertbegin}
	     %   G.insertEdge(u, v) \\
	      %  d[v] = INF
	    %}\label{ricky:BFS3:insertend}
	    %\textbf{end for}\\
	    %BFS($G$, $d$, $src$) \todo{This does not look incremental.} \label{ricky:BFS3:incrbfscall}
	    %}
	%\textbf{\}}
	%\BlankLine
	%\BlankLine
	%\tcc{Decremental BFS}
	\SetKwFunction{FDelete}{DecrementalBFS}
    %\SetKwProg{Pr}{Function}{:}{}
    \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}

	    \Fn{\FDelete{\texttt{Graph} G, \texttt{Graph} BDAG, \texttt{Vertex} src, \texttt{int} dist d[vertex\_n], \texttt{EdgeSet} E'}}{
	    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%	    \Input{$G$ : Base graph}
%	    \Input{$BDAG$ : DAG for base graph}
%	    \Input{$src$ : Source Vertex}
%	    \Input{$d$ : Distance array for each vertex from source}
%	    \Input{$E'$ : Set of Edges in batch update}
	    \BlankLine
	    \texttt{VertexSet} Q1=$\phi$, Q2=$\phi$;\\
	    \For{$((u, v) \in E')\ \textbf{in parallel}$} {\label{ricky:BFS3:delbegin}
	        G.deleteEdge(u, v)\\
	        BDAG.deleteEdge(u, v)\\
	        \textbf{if} $(|v.parent| == 1\ \&\&\ v.parent == u$) $Q_1$.insert(v);
	    }\label{ricky:BFS3:delend}
	    \textbf{end for}\\
	    \While{$(changed)$}{ \label{ricky:BFS2:delloopstart}
	    	changed = 0;\\
	    
	    %\tcc{Algorithm~\ref{ricky:BFS1}}
	    	DeleterHelper(G, BDAG, d, src, E, Q1, Q2); \label{ricky:BFS3:callfun} \\
	    	Q1 = Q2;\\
	    	Q2 = $\phi$;
	    }
	    \textbf{\}}
	    \label{ricky:BFS2:delloopend}\\
	    BFS($G$, $d$, $src$)\label{ricky:BFS2:ricky:BFS3:callBFS}
    }
	\caption{\small \name: Decremental BFS }
	\label{ricky:BFS2}
%	\algstore{BFS}
    \end{algorithm}
 





%\begin{minipage}{.5\linewidth}
%\end{minipage}%
%\begin{minipage}{.5\linewidth}


%\end{minipage}%



==> algorithms/incremental-wcc-gpu.tex <==
\begin{algorithm}[ht]
  \DontPrintSemicolon
  \SetKwFunction{FApplyUnionUpdate}{ApplyUnionUpdate}
  \SetKwProg{Fn}{function}{:}{}

  \SetKwData{VertAdj}{vert\_adjs}
  \SetKwData{ToProcess}{to\_process}
  \SetKwData{VertexN}{vertex\_n}
  \SetKwData{WorkQueue}{work\_queue}
  \SetKwData{VertexN}{vertex\_n}
  \SetKwData{CurrentLane}{current\_lane}
  \SetKwData{Index}{index}
  \SetKwData{Current}{current}
  \SetKwData{Iter}{iter}
  \SetKwData{Last}{last}
  \SetKwData{End}{end}
  \SetKwData{V}{v}
  \SetKwData{LaneMin}{lane\_min}
  \SetKwData{Min}{min\_value}
  \SetKwData{ToUnion}{to\_union}

  \SetKw{True}{true}
  \SetKw{False}{false}
  \SetKw{InvalidVertex}{INVALID\_VERTEX}
  \SetKw{And}{and}

  \SetKwFunction{FnGetVertexAdj}{get\_vertex\_adjacencies}
  \SetKwFunction{FnThreadId}{thread\_id}
  \SetKwFunction{FnLaneId}{lane\_id}
  \SetKwFunction{FnBallotSync}{ballot\_sync}
  \SetKwFunction{FnCurLane}{cur\_lane}
  \SetKwFunction{FnFFS}{ffs}
  \SetKwFunction{FnBegin}{update\_begin}
  \SetKwFunction{FnEnd}{update\_end}
  \SetKwFunction{FnGetPtr}{get\_pointer}
  \SetKwFunction{FnIsValidVertex}{is\_valid\_vertex}
  \SetKwFunction{FnMin}{min}
  \SetKwFunction{FnFindMin}{find\_min}
  \SetKwFunction{FnAtomicMin}{atomicMin}
  \SetKwFunction{FnUnionOp}{union}
  \SetKwFunction{FnFirstLaneId}{first\_lane\_id}

  \Fn() {\FApplyUnionUpdate{\texttt{Graph} G, \texttt{Vertex }Parents[$0\dots vertex\_n$], \texttt{bool} $\ToUnion[0\dots vertex\_n$]}} {
    \texttt{Vertex\_Dictionary}* \VertAdj[] = G.\FnGetVertexAdj{} \;
    \If{((\FnThreadId{} - \FnLaneId{}) \textless \VertexN)}{ \label{unionupdate:eliminate}
      \texttt{bool} \ToProcess \textless ((\FnThreadId{} \textless \VertexN)\ \And \ToUnion[\FnThreadId{}]) \label{unionupdate:enlist}\;
      \texttt{unsigned int32} \WorkQueue = 0 \;
      \While{((\WorkQueue = \FnBallotSync{0xFFFFFFFF, \ToProcess}) $\neq$ 0)} {\label{unionupdate:ballotsync}
        \texttt{int} \CurrentLane = \FnFFS{\WorkQueue} - 1 \label{unionupdate:ffs} \;
        \texttt{int} \Current = (\FnThreadId{} - \FnLaneId{} + \CurrentLane) \label{unionupdate:src} \;
        \texttt{UpdateIterator} \Iter = \VertAdj[\Current].\FnBegin{} \label{unionupdate:iterators_ctor} \;
        \texttt{UpdateIterator} \Last = \VertAdj[\Current].\FnEnd{}  \;
        \While{(\Iter $\neq$ \Last)} { \label{unionupdate:loopstart}
          \V = \InvalidVertex \;
          \If{(\FnLaneId{} $\geq$ \Iter.\FnFirstLaneId{})} { \label{unionupdate:getvertex}
            \V = *\Iter.\FnGetPtr{\FnLaneId{}} \;
          }
          \If{(\FnIsValidVertex{\V})} { \label{unionupdate:check}
            \FnUnionOp{\Current, \V, Parents} \label{unionupdate:unionop} \;
          }
          ++\Iter \label{unionupdate:iterate} \;  
        } \label{unionupdate:loopend}
        \If{(\Index == \FnThreadId{})} {\label{unionupdate:workqueueupdate}
          \ToProcess = \False \label{unionupdate:workqueueend}
        }
      }
    }
  }
  \textbf{end function}
  \caption{Incremental WCC \todo{let's distinguish between the captions of algo 4 and 5.}}
  \label{algorithm:incremental-wcc-optimized}
\end{algorithm}

==> algorithms/iterscheme1_old.tex <==
\begin{algorithm}
  \DontPrintSemicolon
  
  \small
      \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}
  \SetKw{True}{true}
  \SetKw{False}{false}
  \Fn() {IterationScheme1(\texttt{Graph}\ G, \texttt{Vertex} V[vertex\_n])} {
    \texttt{Vertex\_Dictionary}* vert\_adjs[] = G.get\_vertex\_adjacencies() \;
    \If{(thread\_id() - lane\_id() \textless vertex\_n)}{ \label{iteration1:eliminate}
        \texttt{bool} to\_process = (thread\_id() \textless  vertex\_n) %\ ? \True : \False 
        \label{iteration1:toprocess} \;
        \texttt{unsigned int32} work\_queue = 0 \;
        \While{((work\_queue = ballot\_sync(0$\times$FFFFFFFF, to\_process)) $\neq$ 0)} { \label{iteration1:loop-start} \label{iteration1:ballotsync}
          \texttt{int} current\_lane = ffs(work\_queue) - 1 \label{iteration1:ffs}  \;
          \texttt{int} index = (thread\_id() - lane\_id() + current\_lane) \label{iteration1:index} \;
          \texttt{Vertex} src = V[index] \label{iteration1:src} \;
          \tcc{Process source vertex}
          \texttt{SlabIterator} iter = vert\_adjs[src].begin() \label{iteration1:iterators_ctor} \;
          \texttt{SlabIterator} last =  vert\_adjs[src].end() \label{iteration1:iterators_ctor_1} \;
          \tcc{Iterate over adjacent vertices}
          \While{(iter $\neq$ last)} { \label{iteration1:iter-loopstart}
          \texttt{Vertex}  v = *(iter.get\_pointer(lane\_id())) \label{iteration1:getvertex} \;
            \If{(is\_valid\_vertex(v))} { \label{iteration1:check}
              \tcc{Process adjacent vertex}
              \label{iteration1:check-end}
            }
            ++iter \;  \label{iteration1:iter-loopend}
          }
          \tcc{Post-processing}
          \If{(index == thread\_id())} {\label{iteration1:workqueueupdate}
            to\_process = \False \label{iteration1:workqueueend}
          }
        } \label{iteration1:loop-end}
    }
  }
  %\textbf{end function}
    \caption{\small Iteration Scheme 1 (using \texttt{SlabIterator})}
  \label{algorithm:iterscheme1}
\end{algorithm}


==> algorithms/iterscheme3.tex <==
\begin{algorithm}[H]
  \DontPrintSemicolon
  \SetKwFunction{FIterationSchemeTwo}{IterationScheme3}
  \SetKwProg{Fn}{function}{:}{}

  \SetKwData{VertAdj}{vert\_adjs}
  \SetKwData{ToProcess}{to\_process}
  \SetKwData{VertexN}{vertex\_n}
  \SetKwData{WorkQueue}{work\_queue}
  \SetKwData{VertexN}{vertex\_n}
  \SetKwData{CurrentLane}{current\_lane}
  \SetKwData{Index}{index}
  \SetKwData{Current}{current}
  \SetKwData{Iter}{iter}
  \SetKwData{Last}{last}
  \SetKwData{End}{end}
  \SetKwData{V}{v}
  \SetKwData{WarpsN}{warps\_n}
  \SetKwData{GlobalWarpId}{global\_warp\_id}

  \SetKw{True}{true}
  \SetKw{False}{false}

  \SetKwFunction{FnGetVertexAdj}{get\_vertex\_adjacencies}
  \SetKwFunction{FnThreadId}{thread\_id}
  \SetKwFunction{FnLaneId}{lane\_id}
  \SetKwFunction{FnBallotSync}{ballot\_sync}
  \SetKwFunction{FnCurLane}{cur\_lane}
  \SetKwFunction{FnFFS}{ffs}
  \SetKwFunction{FnBegin}{begin}
  \SetKwFunction{FnEnd}{end}
  \SetKwFunction{FnGetPtr}{get\_pointer}
  \SetKwFunction{FnIsValidVertex}{is\_valid\_vertex}


  \Fn() {\FIterationSchemeTwo{$Graph\ G$, $V$, $\VertexN$}} {
    \VertAdj $\leftarrow$ G.\FnGetVertexAdj{} \;
    \WarpsN $\leftarrow$ (blockDim.x * gridDim.x) $\textgreater\textgreater$ 5; \;
    \GlobalWarpId $\leftarrow$ \FnThreadId{} $\textgreater\textgreater$ 5 \;
    i $\leftarrow$ \GlobalWarpId \; \label{iteration2:currentwarpid}

    \While{i $\textless$ \VertexN} {
      \Current $\leftarrow$ V[i] \label{iteration2:currentv} \;
      \tcc{DO: Process source vertex}
      (\Iter, \Last) $\leftarrow$ \VertAdj[\Current].\FnBegin{}, \VertAdj[\Current].\FnEnd{} \label{iteration2:iterators_ctor} \;
      \tcc{Iterate over adjacent vertices}
      \While{$\Iter \neq \Last$} {\label{iteration2:loopstart}
        v $\leftarrow$ *\Iter.\FnGetPtr{\FnLaneId{}} \;
        \If{\FnIsValidVertex{v}} {
          \tcc{DO: Process adjacent vertex} \label{iteration2:loopend}
        }
        ++\Iter \;
      }
      \tcc{DO: Post-processing}
      i += \WarpsN  \label{iteration2:stride} \;
    }
  }
  \caption{Iteration Scheme 2}
  \label{algorithm:iterscheme3}
\end{algorithm}


==> algorithms/pr-compute.tex <==
\begin{algorithm}[H]
  \DontPrintSemicolon
  \small
  \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}  
  \SetKw{True}{true}
  \SetKw{False}{false}
  \SetKw{And}{and}

  \Fn() {ComputePageRank \texttt{(}\texttt{Graph} G,
         \texttt{float} OldPageRanks[VertexN], \texttt{float} NewPageRanks[VertexN],
         \texttt{uint} OutDegrees[VertexN], \texttt{float} damping\_factor), bool frontier[VertexN]\texttt{)}} {
    \texttt{Vertex\_Dictionary}* vert\_adjs[] = G.get\_vertex\_adjacencies() \;
    \If{((thread\_id() - lane\_id()) \textless vertex\_n)} { \label{pagerank:eliminate}
      \texttt{bool} to\_compute = (thread\_id() \textless VertexN) \And frontier[thread\_id()]\label{pagerank:toprocess} \;
      \texttt{float} thread\_local\_value = 0.0f \label{pagerank:local} \;
      \texttt{float} pr\_value = 0.0f \label{pagerank:value} \;
      \texttt{unsigned int32} work\_queue = 0 \;
      \While{$((work\_queue = ballot\_sync(0$\times$FFFFFFFF, to\_process)) \neq 0)$} { \label{pagerank:loop-start} \label{pagerank:ballotsync}
        \texttt{int} current\_lane = ffs(work\_queue) - 1 \label{pagerank:ffs}  \;
        \texttt{int} u = (thread\_id() - lane\_id() + current\_lane) \label{pagerank:src} \;
        thread\_local\_value = 0 \label{pagerank:init-thread-local-value} \;
        \texttt{SlabIterator} iter = vert\_adjs[u].begin() \label{pagerank:iterators_ctor} \;
        \texttt{SlabIterator} last =  vert\_adjs[u].end() \label{pagerank:iterators_ctor_1} \;
         \While{(iter $\neq$ last)} { \label{pagerank:iter-loopstart}
          \texttt{Vertex}  v = *(iter.get\_pointer(lane\_id())) \label{pagerank:getvertex} \;
          \If{(is\_valid\_vertex(v))} { \label{pagerank:check}
            thread\_local\_value += OldPageRanks[v] / OutDegrees[v] \label{pagerank:update-thread-local-value} \;
          }
          ++iter \;  \label{pagerank:iter-loopend}
        }
        i = 1 \label{pagerank:reduce-iter-index-init} \;
        \While{$(i \textless 32)$} { \label{pagerank:reduce-iter-cond}
          thread\_local\_value += shfl\_xor\_sync(0$\times$FFFFFFFF, thread\_local\_value, i) \label{pagerank:reduce-step} \;
          i = i $\times$ 2 \label{pagerank:reduce-iter-index-update} \;
        }        
        thread\_local\_value = shfl\_sync(0$\times$FFFFFFFF, thread\_local\_value) \label{pagerank:broadcast-pr-warp} \;
        \If{$(u == thread\_id())$} {\label{pagerank:workqueueupdate}
          pr\_value = ((1 - damping\_factor) / VertexN) + (damping\_factor * thread\_local\_value) \label{pagerank:apply-damping} \;
          to\_compute = \False \label{pagerank:workqueueend}
        }
      } \label{pagerank:loop-end}
    } 
    \If{(thread\_id() < VertexN)}{
      NewPageRanks[thread\_id()] = frontier[thread\_id()] ? pr\_value : OldPageRanks[thread\_id()] \label{pagerank:new-pr-update} \;
    } 
  }

  \caption{\small PageRank Algorithm - Compute Kernel}
  \label{algorithm:pagerank-compute}
\end{algorithm}


==> algorithms/pr-main.tex <==
\begin{algorithm}[H]
    \small
    \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}  
    \SetKw{True}{true}
    \SetKw{False}{false}
    \SetKw{And}{and}
    \SetKw{Copy}{copy}
  
    \texttt{Graph} in\_graph, out\_graph \label{pagerank:objects} \;
    \tcc{in\_graph and out\_graph store the incoming and outgoing edges for each vertex respectively.} 
    \texttt{Vertex} batch\_src[edge\_n], batch\_dst[edge\_n] \label{pagerank:batch-update} \;
    \texttt{uint} outdegree[vertex\_n], new\_outdegree[vertex\_n] \label{pagerank:outdegrees} \;
    \tcc{For vertex $v$, old\_outdegree[v] is the out-degree in the pre-update graph, and new\_outdegree[v] is
    the out-degree in the post-update graph}
    \texttt{bool} frontier[vertex\_n]  \; 
    \texttt{bool} src[vertex\_n] \;
    \tcc{Initialize \texttt{src}: where, \texttt{src[v] = \True} if v $\in$ \texttt{batch\_src}}. \label{pagerank:frontier}
    \tcc{If batch-insertion, perform here}
    UpdatePageRank(out\_graph, src, old\_pageranks, new\_pageranks, outdegree, new\_outdegree, damping\_factor) \label{pagerank:update-page-rank-1} \;
    \tcc{If batch-deletion, perform here}
    \tcc{Zero-initialize \texttt{frontier}}
    UpdateFrontier(out\_graph, old\_pageranks, new\_pageranks, error\_margin, frontier) \label{pagerank:update-frontier-0} \;
    \Copy out\_degree $\leftarrow$ new\_outdegree \label{pagerank:update-degree} \;
    swap(old\_pageranks, new\_pageranks) \label{pagerank:swap-1} \;
  \While{(\texttt{frontier} has non-\False values)}{ \label{pagerank:condition} 
    ComputePageRank(in\_graph, old\_pageranks, new\_pageranks, damping\_factor, frontier) \label{pagerank:pagerank-compute}\; 
    \tcc{Zero-initialize \texttt{frontier}}
    UpdateFrontier(out\_graph, old\_pageranks, new\_pageranks, error\_margin, frontier) \label{pagerank:update-frontier-2} \; 
    swap(old\_pageranks, new\_pageranks) \label{pagerank:swap-2} \;
  }
    \caption{\small Incremental / Decremental PageRank Algorithm}
    \label{algorithm:pagerank-main}
  \end{algorithm}
  


==> algorithms/pr-update.tex <==
\begin{algorithm}[H]
    \DontPrintSemicolon
    \small
    \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}  
    \SetKw{True}{true}
    \SetKw{False}{false}
    \SetKw{And}{and}
  
    \Fn() {UpdatePageRank \texttt{(}\texttt{Graph} G, \texttt{bool} src\_frontier[VertexN],
           \texttt{float} OldPageRanks[VertexN], \texttt{float} NewPageRanks[VertexN],
           \texttt{uint} OldOutDegrees[VertexN], \texttt{uint} NewOutDegrees[VertexN],
           \texttt{float} damping\_factor\texttt{)}} {
      \texttt{Vertex\_Dictionary}* vert\_adjs[] = G.get\_vertex\_adjacencies() \;
      \If{((thread\_id() - lane\_id()) \textless vertex\_n)} { \label{prupdate:eliminate}
        \texttt{bool} to\_compute = (thread\_id() \textless VertexN) \And src\_frontier[thread\_id()]\label{prupdate:toprocess} \;
        \texttt{unsigned int32} work\_queue = 0 \;
        \While{((work\_queue = ballot\_sync(0$\times$FFFFFFFF, to\_process)) $\neq$ 0)} { \label{prupdate:loop-start} \label{prupdate:ballotsync}
          \texttt{int} current\_lane = ffs(work\_queue) - 1 \label{pagerank:ffs}  \;
          \texttt{int} u = (thread\_id() - lane\_id() + current\_lane) \label{pagerank:src} \;
          \texttt{float} oldpr\_u = shfl\_sync(0$\times$FFFFFFFF, OldPageRanks[u], current\_lane, 32) \label{prupdate:oldpr-u} \;
          \texttt{uint} old\_outdegree\_u = shfl\_sync(0$\times$FFFFFFFF, OldOutDegrees[u], current\_lane, 32) \label{prupdate:oldoutdeg-u} \;
          \texttt{uint} new\_outdegree\_u = shfl\_sync(0$\times$FFFFFFFF, NewOutDegrees[u], current\_lane, 32) \label{prupdate:newoutdeg-u} \;
          \texttt{float} change = damping\_factor $\times$ oldpr\_u $\times$ ((1 / new\_outdegree\_u) - (1 / old\_outdegree\_u)) \label{prupdate:find-change} \;

          \texttt{SlabIterator} iter = vert\_adjs[u].begin() \label{prupdate:iterators_ctor} \;
          \texttt{SlabIterator} last =  vert\_adjs[u].end() \label{prupdate:iterators_ctor_1} \;
           \While{(iter $\neq$ last)} { \label{prupdate:iter-loopstart}
            \texttt{Vertex}  v = *(iter.get\_pointer(lane\_id())) \label{prupdate:getvertex} \;
            \If{(is\_valid\_vertex(v))} { \label{pagerank:check}
              atomicAdd(NewPageRanks[v], change) \label{prupdate:apply-change} \;
            }
            ++iter \;  \label{prupdate:iter-loopend}
          }
          
          \If{(u == thread\_id())} {\label{prupdate:workqueueupdate}
            to\_compute = \False \label{prupdate:workqueueend}
          }
        } \label{prupdate:loop-end}
      } 
    }
  
    \caption{\small PageRank Algorithm - Update Kernel}
    \label{algorithm:pagerank-update}
  \end{algorithm}


==> algorithms/sssp.tex <==
\REM{ 
\begin{algorithm}[H]
    \setcounter{AlgoLine}{0}
	\SetAlFnt{\sffamily}
	\DontPrintSemicolon
	\SetAlgoNoEnd
	\caption{\textsc\textsf{Dynamic SSSP}}
	
	\tcc{SSSP routine modifes $d$ to hold correct distance of each vertex from $src$}
	\SetKwFunction{FMain}{SSSP}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{}}{
	    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	    \SetKwInOut{Requires}{Requires}
	    \SetKwInput{InParallel}{in parallel}
        \SetKwRepeat{Do}{do}{while}
	    \Input{$G$ : Input graph}
	    \Input{$d$ : Distance array for each vertex from source}
	    \Input{$src$ : Source Vertex}
	    \Output{$d$ : Updates the distance array}
	    \BlankLine
	    
	    \Do{$changed$} {
	        $changed \leftarrow false$ \\
	        \For{$u, v \in G.E$ \textbf{in parallel}} {
			\uIf{$d[u] + G.W(u, v) < d[v]$}{\label{ricky:SSSP1:condtion}
	                \BlankLine
                    $d[v] = d[u] + G.W(u, v)$ \\
                    $changed \leftarrow true$
                }
	            \BlankLine
                \textbf{endif}
	        }
	        \BlankLine
	    }
	    \BlankLine
	    
	}
	\textbf{End Function}
	\BlankLine
	\BlankLine
	\caption{SSSP1}
		\label{ricky:SSSP1}
%	\algstore{SSSP}
    \end{algorithm}
    \begin{algorithm} [H]  
%    \algrestore{SSSP}
	
    \setcounter{AlgoLine}{0}
	\SetKwFunction{FHelper}{DELETEHELPER}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FHelper{}}{
	    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	    \SetKwInOut{Requires}{Requires}
	    \SetKwInput{InParallel}{in parallel}
        \SetKwRepeat{Do}{do}{while}
	    \Input{$G$ : Input graph}
	    \Input{$D$ : DAG for base graph}
	    \Input{$d$ : Distance array for each vertex from source}
	    \Input{$src$ : Source Vertex}
	    \Input{$E'$ : Set of Edges in batch update}
	    \Output{$d$ : Updates the distance array}
	    \BlankLine
	    
	    $Q_1 \leftarrow$ empty queue \\
	    $Q_2 \leftarrow$ empty queue \\
	    \For{$u, v \in E'$} {
	        \uIf{$v$ has no other parent in $D$} {
	            $Q_1.insert(v)$ \\
	            $d[v] = INF$
	        }
	    }
	    \BlankLine
	    
	    \Do{$changed$} {
	        $changed \leftarrow false$ \\
	        \For{$u \in Q_1$ \textbf{in parallel}} { 
	            \For{$v \in adj(u, D)$} {
	                \uIf{$v$ has no other parent in $D$ and $d[v] \neq$ INF} {
	                    $d[v] \leftarrow INF$ \\
                        $Q_2.insert(v)$ \\
                        $D.delete(u, v)$ \\
                        $changed \leftarrow true$
                    }
	                \BlankLine
                    \textbf{endif}
                }
	            \BlankLine
	        }
	        
	        $Q_1.clear()$ \\
	        $Q_1.copy(Q_2)$ \\
	        $Q_2.clear()$ \\
	    }
	}
	\BlankLine
	\BlankLine
	
	\tcc{Initialise DAG for base graph $G$}
	$D \leftarrow $ empty graph \\
	\For{$u, v \in G.E$ \textbf{in parallel}} {
	    \uIf{$d[v] == d[u] + G.W(u, v)$}{
	        \BlankLine
            $D.insert(u,v)$
        }
	    \BlankLine
        \textbf{endif}
	}
	\BlankLine
	\BlankLine
	
	\caption{SSSP2}
		\label{ricky:SSSP2}
%    \algstore{SSSP}
    \end{algorithm}
    \begin{algorithm} [H]  
%    \algrestore{SSSP}
	
    \setcounter{AlgoLine}{0}
	\SetKwFunction{FInsert}{INSERTION}
    \SetKwProg{Pr}{Procedure}{:}{}
    \Pr{\FInsert{}}{
	    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	    \Input{$G$ : Base graph}
	    \Input{$src$ : Source Vertex}
	    \Input{$d$ : Distance array for each vertex from source}
	    \Input{$E'$ : Set of Edges in batch update}
	    \BlankLine
	    
	    \For{$u, v \in E'$ \textbf{in parallel}} {
	        $G.insert(u, v)$ \\
	        $d[v] =$ INF
	    }
	    \BlankLine
	    
	    SSSP($G$, $d$, $src$)
	    
	    \BlankLine
    }
	\textbf{End Procedure}
	\BlankLine
	\BlankLine
	
	\SetKwFunction{FDelete}{DELETION}
    \SetKwProg{Pr}{Procedure}{:}{}
    \Pr{\FDelete{}}{
	    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	    \Input{$G$ : Base graph}
	    \Input{$D$ : DAG for base graph}
	    \Input{$src$ : Source Vertex}
	    \Input{$d$ : Distance array for each vertex from source}
	    \Input{$E'$ : Set of Edges in batch update}
	    \BlankLine
	    
	    \For{$u, v \in E'$ \textbf{in parallel}} {
	        $G.delete(u, v)$\\
	        $D.delete(u, v)$
	    }
	    DELETEHELPER($G$, $D$, $d$, $src$)
	    \BlankLine
	    
	    SSSP($G$, $d$, $src$)
	    
	    \BlankLine
    }
	\textbf{End Procedure}
	\BlankLine
	
	\caption{SSSP3}
		\label{ricky:SSSP3}

\end{algorithm}

}

==> algorithms/sssp/create-frontier-decremental.tex <==
\begin{algorithm}[h]
    \DontPrintSemicolon
    \small
    \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}
    \SetKw{True}{true}
    \SetKw{False}{false}
    \SetKw{Return}{return}
    \SetKw{And}{and}
  
    \Fn() {CreateDecrementalFrontier\texttt{(}\texttt{Graph} $G$, \texttt{tree\_node} $D[vertex\_n]$,
      \texttt{Frontier<Edge>} $F$ \texttt{)}} {
      \texttt{Vertex\_Dictionary} *vert\_adjs[] = G.\texttt{get\_vertex\_adjacencies()} \;
      \If{$((thread\_id() - lane\_id())\ \textless\ vertex\_n)$} { \label{frontier-decremental:filter}
        \texttt{bool} to\_consider = $(\texttt{thread\_id()} \textless vertex\_n)\ \And\ (D[\texttt{thread\_id()}].\texttt{distance} \neq \texttt{INVALID})$ \label{frontier-decremental:to-consider} \;
        \texttt{unsigned int32}\ dequeue\_lane = 0 \label{frontier-decremental:init-dequeue-lane} \;
        \While{$((dequeue\_lane = \texttt{warpdequeue}( \&to\_consider)) \neq -1)$} { \label{frontier-decremental:warp-dequeue}
          \texttt{Vertex} current\_v = \texttt{warpbroadcast}(\texttt{thread\_id()}, $dequeue\_lane$) \label{frontier-decremental:current-v} \;
          \texttt{SlabIterator} iter = vert\_adjs[$current\_v$]\texttt{.begin()} \label{frontier-decremental:iter-begin} \;
          \texttt{SlabIterator} last = vert\_adjs[$current\_v$]\texttt{.end()} \label{frontier-decremental:iter-end} \;
          \While{$(iter \neq last)$} { \label{frontier-decremental:loop-start}
            \texttt{Pair} \texttt{p<}$dst, weight$\texttt{>} = \texttt{*(iter.get\_pointer(lane\_id()))} \label{frontier-decremental:get-edge} \;
            \texttt{Edge} $e_{next}$ = \texttt{INVALID\_EDGE} \label{frontier-decremental:init-invalid-edge} \;
            \If{$(is\_valid\_pair(p))$} { \label{frontier-decremental:check-edge}
              $e_{next}$ = \texttt{\{current\_v, p.dst, p.weight\}}\label{frontier-decremental:init-edge}  \;
            }
            \texttt{warpenqeuefrontier}($F, e_{next}, e_{next} \neq \texttt{INVALID\_EDGE}\ \And\ D[p.dst] == $ \texttt{INVALID}) \label{frontier-decremental:enqueue-frontier} \;
            ++ iter \label{frontier-decremental:iter-inc} \; 
          }
        \label{frontier-decremental:loop-end}}
      }
    }
    \caption{Decremental SSSP - Create Frontier}
    \label{algorithm:sssp-frontier-decremental}
  \end{algorithm}


==> algorithms/sssp/init-distance.tex <==
\begin{algorithm}[h]
    \DontPrintSemicolon
    \small
    \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}
    \SetKw{True}{true}
    \SetKw{False}{false}
    \SetKw{Return}{return}
  
    \Fn() {InitializeDistance \texttt{(}\texttt{Vertex} $src$, \texttt{tree\_node} D[vertex\_n]\texttt{)}} {
      \texttt{uint} t = thread\_id() \label{init-dist:init-t} \;
      \If{$(t < vertex\_n)$}{ \label{init-dist:filter-vertex}

          D[t] = $(t == src)$ ? $\left\langle 0, src \right\rangle$ : $\left\langle \texttt{INF}, \texttt{INVALID} \right\rangle$ \label{init-dist:check-edge} \;

      }
    }
    \caption{Static SSSP - Initialize Distance}
    \label{algorithm:sssp-init-distance}
  \end{algorithm}


==> algorithms/sssp/init-frontier-src.tex <==
\begin{algorithm}[h]
    \DontPrintSemicolon
    \small
    \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}
    \SetKw{True}{true}
    \SetKw{False}{false}
    \SetKw{Return}{return}
  
    \Fn() {CreateFrontier \texttt{(}\texttt{Graph} $G$, \texttt{Frontier} F, 
      \texttt{Vertex} src, \texttt{uint} src\_buckets\_n\texttt{)}} {
        \texttt{Vertex\_Dictionary} *vert\_adjs[] = G.\texttt{get\_vertex\_adjacencies()} \;
        \texttt{uint} i = \texttt{global\_warp\_id()} \label{create-frontier:init-counter} \;
        \tcc{Follows IterationScheme2: stride equal to the number of warps}
        \While{$(i < src\_buckets\_n)$} { \label{create-frontier:loop-condition}
          \tcc{Construct BucketIterators for traversing $i^{th}$ slab-list}
          \texttt{BucketIterator} iter = vert\_adjs[$src$]\texttt{.begin\_at(i)} \label{create-frontier:iter-beg} \;
          \texttt{BucketIterator} last = vert\_adjs[$src$]\texttt{.end\_at(i)} \label{create-frontier:iter-end} \;
          \While{$(iter \neq last)$} { \label{create-frontier:loop-begin}
            \texttt{Pair} \texttt{p<}$dst, weight$\texttt{>} = \texttt{*(iter.get\_pointer(lane\_id()))} \label{create-frontier:get-pair} \;
            \texttt{Edge} e = \texttt{INVALID\_EDGE} \label{create-frontier:init-e-invalid} \;
            \If{$(is\_valid\_pair(p))$} { \label{create-frontier:check-valid-pair}
              e = \texttt{\{src, p.dst, p.weight\}} \label{create-frontier:init-edge} \;
            }
            \tcc{Enqueue outgoing edges of source vertex $src$}
            \texttt{warpenqeuefrontier}($F, e, e \neq \texttt{INVALID\_EDGE}$) \label{create-frontier:warp-enqueue-frontier} \;
            ++ iter \label{create-frontier:inc-iter} \;
          }
          i += \texttt{warps\_n()} \label{create-frontier:inc-i} \;
        }
      }
    \caption{Static SSSP - Initialize Frontier}
    \label{algorithm:sssp-init-frontier-src}
  \end{algorithm}



==> algorithms/sssp/set-level-static.tex <==
\begin{algorithm}[h]
  \DontPrintSemicolon
  \small
  \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}
  \SetKw{True}{true}
  \SetKw{False}{false}
  \SetKw{And}{and}
  \SetKw{Return}{return}
  \SetKw{Swap}{swap}
  \SetKwInOut{Input}{input}
  \Input{\ \texttt{Graph} $G$}
  
  \Fn() {BFS\_Kernel\texttt{(}\texttt{Graph} $G$, \texttt{uint} $Level$, \texttt{tree\_node} $D[vertex\_n]$,
    \texttt{Frontier<Edge>} $F_{current}$, \texttt{Frontier<Edge>} $F_{next}$ \texttt{)}} {
    \texttt{Vertex\_Dictionary} *vert\_adjs[] = G.\texttt{get\_vertex\_adjacencies()} \;
    \If{$((thread\_id() - lane\_id())\ \textless\ F_{current}.size)$} { \label{bfs:filter-threads}
      \texttt{Edge} e = \texttt{INVALID\_EDGE} \label{bfs:init} \;
      \texttt{bool} to\_consider = \False \label{bfs:to-consider-init} \;
      \If{$(thread\_id() < F_{current}.size)$}{ \label{bfs:check}
        v = $F_{current}$[\texttt{thread\_id()}] \label{bfs:init-v} \;
        \texttt{tree\_node} \texttt{$d_{src}$} = \texttt{< Level, e.src >} \label{bfs:init-node} \;
        to\_consider = (\texttt{atomicCAS}(\&D[\texttt{e.dst}], \texttt{<INF, INVALID>}, \texttt{<Level, e.src>} ) 
              == \texttt{<INF, INVALID>}) \label{bfs:atomic-cas} \;
      }
      \texttt{unsigned int32}\ dequeue\_lane = 0 \label{bfs:dequeue-lane} \;
      \While{$((dequeue\_lane = \texttt{warpdequeue}( \&to\_consider)) \neq -1)$} { \label{bfs:warp-dequeue}
        \texttt{Vertex} current\_v = \texttt{warpbroadcast}(\texttt{e.dst}, $dequeue\_lane$) \label{bfs:current-v} \;
        \texttt{SlabIterator} iter = vert\_adjs[$current\_v$]\texttt{.begin()} \label{bfs:iter-begin} \;
        \texttt{SlabIterator} last = vert\_adjs[$current\_v$]\texttt{.end()} \label{bfs:iter-end} \;
        \While{$(iter \neq last)$} { \label{bfs:loop-begin}
          \texttt{Vertex} dst = \texttt{*(iter.get\_pointer(lane\_id()))} \label{bfs:fetch-dst} \;
          \texttt{Edge} $e_{next}$= \texttt{INVALID\_EDGE} \label{bfs:init-edge-invalid} \;
          \If{$(is\_valid\_vertex(v))$} { \label{bfs:is-valid-vertex}
            $e_{next}$ = \texttt{\{current\_v, dst\}} \label{bfs:init-edge-next} \;
          }
          \texttt{warpenqeuefrontier}($F_{next}, e_{next}, e_{next} \neq \texttt{INVALID\_EDGE}$) \label{bfs:warp-enqueue} \;
          ++ iter \label{bfs:iterator-inc} \;
        }
      }
    }
  }

  \texttt{Frontier<Edge>} $F_{current}$, $F_{next}$ \label{bfs:create-frontiers} \tcc{Initialize $F_{current}$ and $F_{next}$ with zeroes} 
    \texttt{tree\_node} $nodes[vertex\_n]$ \label{bfs:create-tree-nodes} \tcc{Initialize all elements of nodes with <INF, INVALID>} 
    \texttt{InitializeDistance}(\texttt{SRC}, nodes) \label{bfs:init-distance} \;
    \texttt{CreateFrontier}($G$, $F_{current}$, \texttt{SRC}, $G$.\texttt{get\_bucket\_count()}[\texttt{SRC}]) \label{bfs:create-frontier} \;
    \texttt{uint} $Level$ = 0 \label{bfs:init-level} \;
    \While{$(F_{current}.size \neq 0)$}{ \label{bfs:check-frontier-size}
      \texttt{BFS\_Kernel}($G$, $Level$, $nodes$, $F_{current}$, $F_{next}$) \label{bfs:run-bfs} \;
      \Swap $F_{current}$ $F_{next}$ \label{bfs:swap} \;
      ++ Level \label{bfs:increment-level} \;
    }
  \caption{Static Level-based Breadth First Search}
  \label{algorithm:bfs-set-level-static}
\end{algorithm}


==> algorithms/tc-slabgraph.tex <==
\begin{algorithm}
    \setcounter{AlgoLine}{0}
	\SetAlFnt{\sffamily}
	\DontPrintSemicolon
	\SetAlgoNoEnd

    \SetKwFunction{FMain}{COUNT}
 %   \SetKwProg{Fn}{Function}{:}{}
 \SetKwProg{Fn}{Function}{\{}{\}}

    \Fn{\FMain{ \texttt{Graph} $G_{1}$,\texttt{Graph} $G_{2}$, \texttt{EdgeSet} E', \texttt{int} $T$[$vertex_{n}$], \texttt{int} m }}{
	    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	    \SetKwInOut{Requires}{Requires}
	    \SetKwInput{InParallel}{in parallel}
	%    \Input{$G_1, G_2$ : Input graphs}
	 %   \Input{$E'$ : Set of Edges in batch update}
	  %  \Input{$m$: Integer factor}
	  %  \Output{$T_n$ : Per vertex Triangle array}
	    \BlankLine

	    $totalcount$ = $0$\\
	    \BlankLine

	    \For{($u, v \in E'$ \textbf{in parallel})} {\label{algotccount:foronebegin}
	        $count$ = $0$\\
    	    \texttt{Vertex} vert\_adjs[] = G1.get\_vertex\_adjacencies()\\
 
            \texttt{SlabIterator} iter = vert\_adjs[u].begin()\\
            \texttt{SlabIterator} last = vert\_adjs[u].end()\\
 
            /* Iterate over adjacent vertices */\\
            \While{ (iter != last)}{\label{algotccount:whilebegin}
                    \texttt{Vertex} w = *(iter.get\_pointer(lane\_id()))\\
			        \If{( $G_1$.SearchEdge(u,w)\&\& $G_2$.SearchEdge(w,u) )}{
				        count=count + 1\\
                        $T[w]$ = $T[w]$ + m\\
                    }
                    \textbf{end if}\\
            }
            \textbf{end while}\label{algotccount:whileend}\\
        $T[u]$ = $T[u]$ + m $\times$count\\
      $T[v]$ = $T[v]$ + m $\times$ count\\
      totalcount = totalcount + 3 $\times$ count\\
}
\textbf{end for}\label{algotccount:foroneend}\\
\texttt{return} totalcount \\%\textcolor{brown}{COUNT Function in  Algorithm~\ref{ricky:algotc} can be removed?}\\
}
%\textbf{End Function}
\caption{\textsc\textsf{Count Function: \name code}}
	\label{slabgraph:tccount}

\end{algorithm}
	

==> algorithms/work-cooperative.tex <==
\begin{algorithm}[t]
  \DontPrintSemicolon
  \SetKwFunction{FSearchWCWS}{SearchWCWS}
 % \SetKwProg{Fn}{function}{:}{}
\SetKwProg{Fn}{}{\{}{\}}
  \SetKwData{VertAdj}{vert\_adjs}
  \SetKwData{ToProcess}{to\_process}
  \SetKwData{VertexN}{vertex\_n}
  \SetKwData{WorkQueue}{work\_queue}
  \SetKwData{PrevWorkQueue}{prev\_work\_queue}
  \SetKwData{VertexN}{vertex\_n}
  \SetKwData{CurrentLane}{current\_lane}
  \SetKwData{Index}{index}
  \SetKwData{Current}{current}
  \SetKwData{Iter}{iter}
  \SetKwData{Last}{last}
  \SetKwData{End}{end}
  \SetKwData{V}{v}
  \SetKwData{WarpsN}{warps\_n}
  \SetKwData{GlobalWarpId}{global\_warp\_id}
  \SetKwData{BucketVertex}{bucket\_vertex}
  \SetKwData{BucketIndex}{bucket\_index}
  \SetKwData{Src}{src}
  \SetKwData{Index}{index}
  \SetKwData{ToSearch}{to\_search}
  \SetKwData{Key}{key}
  \SetKwData{Found}{found}
  \SetKwData{CurSlab}{current\_slab}
  \SetKwData{SrcLane}{src\_lane}
  \SetKwData{CurrentVertex}{cur\_vertex}
  \SetKwData{Bucket}{bucket}
  \SetKwData{LaneValue}{lane\_value}
  \SetKwData{BitSet}{bitset}
  \SetKwData{LaneFound}{lane\_found}
  \SetKwData{Found}{found}
  \SetKwData{Ptr}{ptr}

  \SetKw{DeviceFn}{\_\_device\_\_}
  \SetKw{True}{true}
  \SetKw{False}{false}
  \SetKw{HeadSlab}{HEAD\_SLAB}
  \SetKw{Nullptr}{nullptr}

  \SetKwFunction{FnGetVertexAdj}{get\_vertex\_adjacencies}
  \SetKwFunction{FnThreadId}{thread\_id}
  \SetKwFunction{FnLaneId}{lane\_id}
  \SetKwFunction{FnBallotSync}{ballot\_sync}
  \SetKwFunction{FnShuffleSync}{shuffle\_sync}
  \SetKwFunction{FnCurLane}{cur\_lane}
  \SetKwFunction{FnFFS}{ffs}
  \SetKwFunction{FnBegin}{begin\_at}
  \SetKwFunction{FnEnd}{end\_at}
  \SetKwFunction{FnGetPtr}{get\_pointer}
  \SetKwFunction{FnIsValidVertex}{is\_valid\_vertex}
  \SetKwFunction{FnHash}{hash}
  \SetKwFunction{FnReadSlab}{read\_slab}
  \SetKwFunction{FnIsKeyLane}{is\_key\_lane}

    \small
  \Fn() { \FSearchWCWS{$\ToSearch$, $\Key$, $\Found$}} {
    \CurSlab = \HeadSlab \;
    \WorkQueue= \FnBallotSync{\ToSearch} \label{search:workqueue} \;
    \PrevWorkQueue = \WorkQueue \label{search:prevworkqueue} \;
    \While{\WorkQueue $\neq$ 0} {\label{search:checkworkqueue}
      \CurSlab =  (\WorkQueue $\neq$ \PrevWorkQueue) ? \CurSlab\ : \HeadSlab \label{search:previouskeyfound} \;
      \SrcLane = \FnFFS{\WorkQueue} - 1 \label{search:nextlane} \;
      \CurrentVertex = \FnShuffleSync{\Key, \SrcLane} \label{search:curvertex} \;
      \Bucket = \FnHash{\CurrentVertex} \label{search:findbucket} \;
      \LaneValue = \FnReadSlab{\FnLaneId{}, \CurSlab} \label{search:findlanevalue} \;
      \BitSet = \FnBallotSync{\Key == \LaneValue} \label{search:findmatchbitset1} \;
      \LaneFound = \FnFFS{\BitSet} - 1 \label{search:findmatchbitset2} \;
      \uIf{\FnIsKeyLane{\LaneFound}} { \label{search:foundkey}
        \If{\FnLaneId{} == \SrcLane} {
          \ToSearch = \False \label{search:updateworkqueue1} \;
        }
      } \Else {
        \Ptr = \FnShuffleSync{\LaneValue, 31} \label{search:shflnextptr} \;
        \uIf{\Ptr == \Nullptr} {
          \If{\FnLaneId{} == \SrcLane} {\label{search:endslablist1}
            \Found = \False \;
            \ToSearch = \False \label{search:endslablist2} \;
          }
        } \Else {
          \CurSlab = \Ptr \;
        }
      }
      \WorkQueue = \FnBallotSync{to\_search} \label{search:updateworkqueue2} \;
    }
  }
%  \textbf{end function}
  \caption{\hl{\small Warp-cooperative strategy: Search}}
  \label{algo:WCWS}
\end{algorithm}


==> experimental-plots/pagerank/plots/PR-dec-large.tex <==

\pgfplotsset{
  time-large/.style={
    legend style={draw=none, font=\small},
    legend cell align=left,
    ylabel style={align=center, font=\bfseries\boldmath},
    xlabel style={align=center, font=\bfseries\boldmath},
    xtick={1,2,3,4},
    xticklabels={1K,10K,100K,1000K},
    xtick distance=1,
    xlabel={Batch Size (K = $10^3$)},
    y tick label style={/pgf/number format/.cd, set thousands separator={}},
    scaled ticks=false,
    every axis plot/.append style={thick},
  },
}

\begin{figure}
\centering
  \begin{tabular}[c]{ccc}

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Higgs}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Higgs-decremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Higgs-decremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Higgs-decremental-time-large}
  
\end{subfigure} &     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Orkut}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Orkut-decremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Orkut-decremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Orkut-decremental-time-large}
  
\end{subfigure} &     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\USAfull}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-USAfull-decremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/USAfull-decremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-USAfull-decremental-time-large}
  
\end{subfigure} \\ \vspace{-5pt}     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Lj}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Lj-decremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Lj-decremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Lj-decremental-time-large}
  
\end{subfigure} &     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Pokec}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Pokec-decremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Pokec-decremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Pokec-decremental-time-large}
  
\end{subfigure} &     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Randtenm}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Randtenm-decremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Randtenm-decremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Randtenm-decremental-time-large}
  
\end{subfigure} \\ \vspace{-5pt}     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\BerkStan}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-BerkStan-decremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/BerkStan-decremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-BerkStan-decremental-time-large}
  
\end{subfigure} &     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Wikipedia}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Wikipedia-decremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Wikipedia-decremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Wikipedia-decremental-time-large}
  
\end{subfigure} &     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Wikitalk}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Wikitalk-decremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Wikitalk-decremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Wikitalk-decremental-time-large}
  
\end{subfigure} \\ \vspace{-5pt}     
  
  \end{tabular}
 \caption{\small{\textsc{PageRank }(\textsc{decremental} - \textsc{large batches})}}
 \label{plot:PageRank-time-large-decremental}
\end{figure}


==> experimental-plots/pagerank/plots/PR-inc-large.tex <==

\pgfplotsset{
  time-large/.style={
    legend style={draw=none, font=\small},
    legend cell align=left,
    ylabel style={align=center, font=\bfseries\boldmath},
    xlabel style={align=center, font=\bfseries\boldmath},
    xtick={1,2,3,4},
    xticklabels={1K,10K,100K,1000K},
    xtick distance=1,
    xlabel={Batch Size (K = $10^3$)},
    y tick label style={/pgf/number format/.cd, set thousands separator={}},
    scaled ticks=false,
    every axis plot/.append style={thick},
  },
}

\begin{figure}
\centering
  \begin{tabular}[c]{ccc}

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Higgs}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Higgs-incremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Higgs-incremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Higgs-incremental-time-large}
  
\end{subfigure} &     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Orkut}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Orkut-incremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Orkut-incremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Orkut-incremental-time-large}
  
\end{subfigure} &     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\USAfull}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-USAfull-incremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/USAfull-incremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-USAfull-incremental-time-large}
  
\end{subfigure} \\ \vspace{-5pt}     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Lj}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Lj-incremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Lj-incremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Lj-incremental-time-large}
  
\end{subfigure} &     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Pokec}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Pokec-incremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Pokec-incremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Pokec-incremental-time-large}
  
\end{subfigure} &     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Randtenm}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Randtenm-incremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Randtenm-incremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Randtenm-incremental-time-large}
  
\end{subfigure} \\ \vspace{-5pt}     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\BerkStan}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-BerkStan-incremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/BerkStan-incremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-BerkStan-incremental-time-large}
  
\end{subfigure} &     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Wikipedia}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Wikipedia-incremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Wikipedia-incremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Wikipedia-incremental-time-large}
  
\end{subfigure} &     
  

\begin{subfigure}{0.3\textwidth}
  \begin{tikzpicture}[scale = 0.55]

    \begin{axis}[time-large,y axis line style=blue,axis y line*=right,axis x line=none,ylabel=Iterations,title={\textsc{\Wikitalk}}]
      \addplot+[mark=o,blue] table[x=batch,y=iterations, col sep=comma] {plot-data/iter-Wikitalk-incremental-large.csv};
    \end{axis}

    \begin{axis}[time-large,y axis line style=red,axis y line*=left,ylabel=Avg. Running Time (in ms.)]
      \addplot+[mark=x,red] table[x=batch,y=time, col sep=comma] {plot-data/Wikitalk-incremental-large.csv};
    \end{axis}
\end{tikzpicture} 
  \label{plot:PageRank-Wikitalk-incremental-time-large}
  
\end{subfigure} \\ \vspace{-5pt}     
  
  \end{tabular}
 \caption{\small{\textsc{PageRank }(\textsc{incremental} - \textsc{large batches})}}
 \label{plot:PageRank-time-large-incremental}
\end{figure}


==> main.tex <==
Among\begin{algorithm}[h]
    \DontPrintSemicolon
    \small
    \SetKwProg{Fn}{\FnKeyword}{\ \{}{\}}
    \SetKw{True}{true}
    \SetKw{False}{false}
    \SetKw{Return}{return}
    \SetKw{Swap}{swap}
    \SetKwInOut{Input}{input}
    \Input{\ \texttt{Graph} $G$, \texttt{EdgeBatches} $batches$[$batch\_n$]}
    \tcc{Static SSSP}  
    \texttt{Frontier<Edge>} $F_{current}$, $F_{next}$ \label{sssp-main:init-frontier} \tcc{Initialize $F_{current}$ and $F_{next}$ with zeroes} 
    \texttt{tree\_node} $nodes[vertex\_n]$ \label{sssp-main:init-tree-nodes} \tcc{Initialize all elements of nodes with <INF, INVALID>} 
    \texttt{InitializeDistance}(\texttt{SRC}, nodes) \label{sssp-main:init-distance} \;
    \texttt{CreateFrontier}($G$, $F_{current}$, \texttt{SRC}, $G$.\texttt{get\_bucket\_count()}[\texttt{SRC}]) \label{sssp-main:create-frontier} \;
    \While{$(F_{current}.size \neq 0)$}{ \label{sssp-main:check-static-frontier-size}
      \texttt{SSSP\_Kernel}(G, nodes, $F_{current}$, $F_{next}$) \label{sssp-main:kernel} \;
      \Swap ($F_{current}$, $F_{next}$) \label{sssp-main:swap-frontier-static} \;
    }
    \tcc{Dynamic SSSP}
    \tcc{Initialize $F_{current}$ and $F_{next}$ with zeroes} 
    \For{b \textbf{in} batches}{ \label{sssp-main:for-loop}
      \If{$(b.\texttt{is\_insertion()})$} { \label{sssp-main:check-is-insertion}
        \textbf{\textit{Incremental Algorithm Prologue:}} \;
        \tcc{Insert batch of edges $b$ into $G$}
        \tcc{Initialize $F_{current}$ with the batch of edges in $b$}
        \texttt{SSSP\_Kernel}(G, nodes, $F_{current}$, $F_{next}$) \label{sssp-main:kernel-batch} \;
        \Swap ($F_{current}$, $F_{next}$) \label{sssp-main:swap-frontier-incremental} \;
      } \Else {
        \textbf{\textit{Decremental Algorithm Prologue:}} \;
        \tcc{Delete batch of edges $b$ from $G$}
        \texttt{Invalidate}(b.edges, nodes) \label{sssp-main:invalidate} \;
        \texttt{PropogateInvalidation}(nodes, \texttt{SRC}) \label{sssp-main:proppogate-invalidation} \;
        \tcc{Initialize $F_{current}$ and $F_{next}$ with zeroes} 
        \texttt{CreateDecrementalFrontier}($G$, nodes, $F_{current}$) \label{sssp-main:create-dec-frontier} \;
      }
      \textbf{\textit{Common Epilogue:}} \;
      \While{$(F_{current}.size \neq 0)$}{ \label{sssp-main:check-frontier-size-dynamic}
        \texttt{SSSP\_Kernel}(G, nodes, $F_{current}$, $F_{next}$) \label{sssp-main:kernel-dynamic} \;
        \Swap ($F_{current}$, $F_{next}$) \label{sssp-main:swap-frontier-dynamic} \;
      }
    }

    \caption{SSSP - Incremental / Decremental}
    \label{algorithm:sssp-main}
  \end{algorithm}

==> tables/bfs-decremental-large.tex <==
\begin{table}[h]
  \small
  \centering
  
  \begin{tabular}{lrrrr}
    \hline
    \multirow{2}{*}{Graph} & \multicolumn{4}{c}{Incremental Update Batch Size ($K = 10^3$)} \\\cline{2-5}
    & 1K & 10K & 100K & 1000K \\
    \hline
    \Higgs & 3.101 & 3.099 & 3.094 & 4.431 \\
    \Orkut & 20.235 & 20.458 & 20.448 & 30.182 \\
    \USAfull & 1279.874 & 1212.865 & 590.237 & 1448.46 \\
    \Lj & 39.137 & 39.395 & 39.162 & 58.284 \\
    \Pokec & 17.567 & 17.405 & 17.106 & 24.822 \\
    \Randtenm & 109.177 & 106.696 & 104.191 & 156.756 \\
    \BerkStan & 18.013 & 17.972 & 11.795 & 9.463 \\
    \Wikipedia & 41.487 & 41.574 & 34.037 & 42.449 \\
    \Wikitalk & 10.639 & 10.158 & 9.449 & 11.096 \\
    \hline
  \end{tabular}

  \caption{BFS Decremental: Performance of decremental batch updates performed on the full graph. Execution time in ms.}
  \label{table:bfs-decremental-large}
\end{table}

==> tables/bfs-decremental-small.tex <==
\begin{table}[h]
  \small
  \centering

  \begin{tabular}{lrrrrrrrrrr}
    \hline
    \multirow{2}{*}{Graph}  & \multicolumn{10}{c}{Incremental Update Batch Size ($K = 10^3$)} \\\cline{2-11}
    & 1K  & 2K  & 3K  & 4K  & 5K  & 6K  & 7K  & 8K  & 9K  & 10K \\
    \hline
    \Higgs & 3.11 & 3.111 & 3.122 & 3.123 & 3.118 & 3.101 & 3.116 & 3.136 & 3.126 & 3.122 \\
    \Orkut & 19.303 & 19.327 & 19.349 & 19.371 & 19.48 & 19.397 & 19.636 & 19.454 & 19.456 & 19.794 \\
    \USAfull & 591.448 & 420.183 & 476.672 & 388.689 & 397.562 & 329.081 & 357.427 & 341.232 & 375.261 & 370.814 \\
    \Lj & 36.946 & 38.141 & 39.536 & 39.95 & 40.055 & 39.661 & 39.745 & 39.691 & 40.145 & 39.784 \\
    \Pokec & 17.598 & 17.466 & 16.818 & 17.041 & 17.338 & 16.849 & 16.424 & 16.761 & 17.211 & 17.252 \\
    \Randtenm & 110.591 & 109.44 & 104.634 & 110.397 & 110.424 & 110.151 & 110.286 & 109.811 & 109.984 & 109.889 \\
    \BerkStan & 9.712 & 9.353 & 8.102 & 7.661 & 7.04 & 7.174 & 6.454 & 6.722 & 6.423 & 6.263 \\
    \Wikipedia & 41.286 & 41.411 & 41.515 & 41.487 & 41.424 & 37.008 & 34.868 & 41.871 & 41.552 & 41.086 \\
    \Wikitalk & 9.791 & 9.94 & 10.376 & 9.962 & 9.947 & 9.939 & 9.999 & 9.94 & 10.779 & 10.008 \\
    \hline
  \end{tabular}
      
  \caption{SSSP Decremental: Performance of decremental batch updates in ms.}
  \label{table:bfs-decremental-small}
\end{table}

==> tables/bfs-incremental-large.tex <==
\begin{table}[h]
  \small
  \centering

  \begin{tabular}{lrrrr}
    \hline
    \multirow{2}{*}{Graph} & \multicolumn{4}{c}{Incremental Update Batch Size ($K = 10^3$)} \\\cline{2-5}
    & 1K & 10K & 100K & 1000K \\
    \hline
    \Higgs & 0.406 & 0.627 & 1.274 & 3.516 \\
    \Orkut & 1.205 & 1.508 & 1.606 & 15.119 \\
    \USAfull & 750.987 & 603.876 & 351.711 & 151.2 \\
    \Lj & 0.72 & 2.888 & 8.385 & 36.971 \\
    \Pokec & 0.599 & 2.035 & 4.277 & 20.141 \\
    \Randtenm & 12.125 & 19.818 & 19.849 & 81.508 \\
    \BerkStan & 1.203 & 0.692 & 2.006 & 3.682 \\
    \Wikipedia & 5.39 & 8.759 & 7.326 & 30.049 \\
    \Wikitalk & 0.757 & 0.474 & 1.471 & 10.261 \\
    \hline
  \end{tabular}

  \caption{BFS Incremental: Performance of incremental batch updates performed on 75\% of original graph. Execution time in ms.}
  \label{table:bfs-incremental-large}
\end{table}

==> tables/bfs-incremental-small.tex <==
\begin{table}[h]
  \small
  \centering

  \begin{tabular}{lrrrrrrrrrr}
    \hline
    \multirow{2}{*}{Graph}  & \multicolumn{10}{c}{Incremental Update Batch Size ($K = 10^3$)} \\\cline{2-11}
    & 1K  & 2K  & 3K  & 4K  & 5K  & 6K  & 7K  & 8K  & 9K  & 10K \\
    \hline
    \Higgs & 1.085 & 1.036 & 0.964 & 0.92 & 0.924 & 0.955 & 0.906 & 0.903 & 0.941 & 0.924 \\
    \Orkut & 0.352 & 0.38 & 0.417 & 0.421 & 0.757 & 0.585 & 0.736 & 0.73 & 0.677 & 0.702 \\
    \USAfull & 203.637 & 186.299 & 197.562 & 184.723 & 184.478 & 199.564 & 189.609 & 174.851 & 178.527 & 174.179 \\
    \Lj & 7.916 & 7.686 & 7.87 & 7.763 & 7.992 & 8.156 & 8.013 & 8.263 & 8.188 & 8.093 \\
    \Pokec & 4.593 & 4.009 & 4.079 & 4.038 & 4.345 & 4.383 & 4.216 & 4.26 & 4.29 & 4.306 \\
    \Randtenm & 14.489 & 15.821 & 16.255 & 19.507 & 19.263 & 20.85 & 19.758 & 21.879 & 18.257 & 21.406 \\
    \BerkStan & 10.839 & 8.339 & 6.022 & 5.047 & 4.485 & 4.19 & 4.437 & 3.138 & 3.302 & 2.763 \\
    \Wikipedia & 8.153 & 7.072 & 7.545 & 8.564 & 8.299 & 8.358 & 8.002 & 7.955 & 8.483 & 7.595 \\
    \Wikitalk & 1.737 & 2.02 & 2.02 & 2.479 & 2.488 & 2.396 & 2.062 & 1.743 & 1.994 & 2.007 \\
    \hline
  \end{tabular}
  
  \caption{BFS Incremental: Performance of incremental batch updates in ms.}
  \label{table:bfs-incremental-small}
\end{table}

==> tables/bfs-static.tex <==
\begin{table}[h]
  \small
  \centering

  \begin{tabular}{lrrr}\hline
    Graph & Hornet & \name & \name (tree) \\
    \hline
    \Higgs & 2.28 & 2.247 & 2.924 \\
    \Orkut & 78.557 & 85.674 & 122.716 \\
    \USAfull & 660.058 & 237.233 & 240.221 \\
    \Lj & 25.337 & 30.29 & 36.114 \\
    \Pokec & 8.37 & 10.116 & 14.895 \\
    \Randtenm & 77.218 & 80.172 & 84.747 \\
    \BerkStan & 30.865 & 14.343 & 14.438 \\
    \Wikipedia & 28.392 & 26.057 & 33.45 \\
    \Wikitalk & 4.934 & 8.234 & 9.191 \\
    \hline
  \end{tabular}
      
  \caption{BFS Static: Hornet vs. \name. Execution time in ms.}
  \label{table:bfs-static}
\end{table}

==> tables/graphdelete-bulk.tex <==
\begin{table}[h]
  \centering
  \small
  \begin{tabular}{lrrr}\hline
    Graph &  \textsc{Stinger (CPU)} & \textsc{Hornet (GPU)} & \textsc{\SG (GPU)} \\\hline
    \Higgs & 63.2566 & 277.206 & 443.754 \\
    \Orkut & 98.9557 & 40.2771 & 346.237 \\
    \USAfull & 68.7894 & 26.52 & 325.748 \\
    \Lj & 68.6722 & 157.327 & 349.177 \\
    \Pokec & 56.6961 & 194.702 & 365.314 \\
    \Randtenm & 33.6571 & 1412.23 & 432.866 \\
    \BerkStan & 103.86 & 125.28 & 2215.72 \\
    \Wikipedia & 67.9179 & 259.511 & 360.211 \\
    \Wikitalk & 31.7002 & 265.26 & 2355.89 \\
    \hline
  \end{tabular}
  \caption{Bulk Delete Benchmark (in millions of edges per second)}
  \label{tab:graphdelete-bulk}
\end{table}

==> tables/graphdelete.tex <==
\begin{table}[h]
    \centering
    \small
    \setlength{\tabcolsep}{3,2pt}
    \resizebox{\textwidth}{!}{\begin{tabular}{llrrrrrrrrrrr}\hline
        \multirow{2}{*}{Data Structure} & \multirow{2}{*}{Graph} & \multicolumn{10}{c}{Batch Deletion (K = $10^3$)} \\\cline{3-12}
        &  & 1K & 2K & 3K & 4K & 5K & 6K & 7K & 8K & 9K & 10K \\ \hline
        \multirow{9}{*}{\textsc{Hornet (GPU)}} & \Higgs & 1.917 & 3.751 & 5.714 & 7.24 & 5.52 & 6.621 & 5.454 & 6.233 & 9.557 & 10.531 \\
        & \Orkut & 1.771 & 3.572 & 5.342 & 7.005 & 5.61 & 6.695 & 7.953 & 9.15 & 10.172 & 11.246 \\
        & \USAfull & 1.93 & 3.755 & 5.521 & 6.887 & 5.796 & 6.57 & 7.455 & 8.065 & 8.361 & 9.052 \\
        & \Lj & 1.881 & 3.675 & 5.265 & 6.858 & 5.496 & 6.351 & 7.351 & 7.689 & 8.784 & 10.031 \\
        & \Pokec & 1.878 & 3.693 & 5.516 & 7.055 & 5.49 & 6.4 & 7.338 & 8.273 & 8.994 & 10.186 \\
        & \Randtenm & 2.063 & 4.135 & 6.183 & 8.099 & 6.731 & 7.954 & 9.285 & 10.476 & 11.683 & 12.874 \\
        & \BerkStan & 1.882 & 3.664 & 5.479 & 6.982 & 5.452 & 6.408 & 7.466 & 8.203 & 8.851 & 9.776 \\
        & \Wikipedia & 2.009 & 4.001 & 5.911 & 7.548 & 6.462 & 7.475 & 8.497 & 9.686 & 10.064 & 11.149 \\
        & \Wikitalk & 1.947 & 3.922 & 5.68 & 7.381 & 5.92 & 6.73 & 7.582 & 8.765 & 9.749 & 10.066 \\
        \hline
        \multirow{9}{*}{\textsc{\SG (GPU)}} & \Higgs & 18.327 & 37.043 & 54.143 & 69.829 & 85.249 & 101.249 & 113.816 & 128.302 & 136.761 & 148.074 \\
        & \Orkut & 21.918 & 43.932 & 63.496 & 82.357 & 97.719 & 111.295 & 127.491 & 144.134 & 149.706 & 160.519 \\
        & \USAfull & 22.2 & 44.071 & 63.635 & 80.857 & 97.295 & 111.27 & 126.516 & 140.62 & 149.808 & 159.393 \\
        & \Lj & 21.121 & 41.762 & 59.251 & 77.028 & 93.341 & 109.747 & 123.411 & 138.932 & 144.734 & 158.451 \\
        & \Pokec & 17.909 & 36.177 & 52.66 & 69 & 81.714 & 98.222 & 109.496 & 121.523 & 129.307 & 140.203 \\
        & \Randtenm & 18.353 & 36.933 & 54.049 & 70.455 & 84.378 & 100.747 & 113.047 & 127.822 & 131.564 & 146.064 \\
        & \BerkStan & 21.793 & 42.681 & 63.339 & 80.16 & 95.712 & 109.667 & 127.24 & 135.531 & 145.82 & 157.881 \\
        & \Wikipedia & 21.825 & 43.578 & 63.786 & 80.823 & 97.246 & 113.598 & 127.91 & 142.648 & 150.534 & 162.375 \\
        & \Wikitalk & 18.318 & 37.387 & 53.926 & 73.09 & 83.914 & 104.105 & 117.337 & 132.663 & 138.253 & 152.409 \\
        \hline
    \end{tabular}}
    \caption{Deletion benchmark (in millions of edges per second )}
    \label{tab:deletion-benchmark}
\end{table}


==> tables/graphinsert.tex <==
\begin{table}[h]
    \centering
    \small
    \setlength{\tabcolsep}{3.2pt}
    \resizebox{\textwidth}{!}{\begin{tabular}{llrrrrrrrrrrrr}\hline
        \multirow{2}{*}{Data Structure} &  \multirow{2}{*}{Graph} &  \multirow{2}{*}{Bulk Insert} &  \multicolumn{10}{c}{Batch Insert (K = $10^3$)} \\\cline{4-13}
        &   &   &  1K &  2k &  3K &  4K &  5K &  6K &  7K &  8K &  9K &  10K \\\hline 
        \multirow{9}{*}{\textsc{Stinger (CPU)}} & \Higgs & 0.978 & 0.171 & 0.233 & 0.307 & 0.327 & 0.345 & 0.358 & 0.371 & 0.396 & 0.357 & 0.409 \\
        & \Orkut & 0.204 & 0.189 & 0.202 & 0.211 & 0.232 & 0.332 & 0.356 & 0.407 & 0.186 & 0.406 & 0.407 \\
        & \USAfull & 0.882 & 0.651 & 0.726 & 0.768 & 0.777 & 0.804 & 0.801 & 0.815 & 0.85 & 0.852 & 0.904 \\
        & \Lj & 1.314 & 0.55 & 0.553 & 0.577 & 0.59 & 0.592 & 0.621 & 0.599 & 0.61 & 0.605 & 0.643 \\
        & \Pokec & 0.176 & 0.214 & 0.211 & 0.208 & 0.242 & 0.423 & 0.407 & 0.407 & 0.436 & 0.535 & 0.509 \\
        & \Randtenm & 0.111 & 0.112 & 0.112 & 0.111 & 0.115 & 0.117 & 0.119 & 0.122 & 0.12 & 0.121 & 0.12 \\
        & \BerkStan & 1.074 & 0.178 & 0.175 & 0.247 & 0.254 & 0.296 & 0.334 & 0.331 & 0.348 & 0.358 & 0.379 \\
        & \Wikipedia & 0.982 & 0.084 & 0.128 & 0.15 & 0.162 & 0.207 & 0.208 & 0.225 & 0.197 & 0.233 & 0.263 \\
        & \Wikitalk & 0.096 & 0.112 & 0.158 & 0.18 & 0.184 & 0.189 & 0.177 & 0.245 & 0.263 & 0.33 & 0.284 \\
        \hline
        \multirow{9}{*}{\textsc{Hornet (GPU)}} & \Higgs & 316.826 & 3.826 & 7.811 & 11.421 & 14.264 & 8.2 & 9.773 & 6.891 & 8.252 & 14.282 & 15.796 \\
        & \Orkut & 38.077 & 4.029 & 8.662 & 12.499 & 15.695 & 8.845 & 10.64 & 12.523 & 14.435 & 16.175 & 17.776 \\
        & \USAfull & 36.106 & 3.242 & 5.525 & 7.043 & 8.262 & 6.202 & 7.238 & 8.785 & 10.345 & 11.99 & 12.53 \\
        & \Lj & 212.177 & 3.632 & 6.961 & 9.324 & 11.562 & 7.06 & 8.26 & 9.752 & 10.877 & 12.501 & 14.46 \\
        & \Pokec & 245.584 & 3.815 & 7.442 & 10.493 & 13.07 & 7.526 & 8.916 & 10.553 & 11.987 & 13.394 & 14.991 \\
        & \Randtenm & 88.73 & 4.126 & 8.431 & 12.053 & 15.132 & 9.689 & 11.42 & 13.275 & 14.974 & 16.941 & 18.589 \\
        & \BerkStan & 141.098 & 3.7 & 7.123 & 9.438 & 12.029 & 7.477 & 8.901 & 10.559 & 11.919 & 13.226 & 14.804 \\
        & \Wikipedia & 526.466 & 3.946 & 7.549 & 10.492 & 12.395 & 8.265 & 9.822 & 11.805 & 13.206 & 15.206 & 16.803 \\
        & \Wikitalk & 425.679 & 4.171 & 8.501 & 11.976 & 13.408 & 8.817 & 11.358 & 10.47 & 12.351 & 15.386 & 15.923 \\
        \hline
        \multirow{9}{*}{\textsc{\SG (GPU)}} & \Higgs & 1832.7 & 12.825 & 33.602 & 51.676 & 66.237 & 79.247 & 94.865 & 107.467 & 122.147 & 134.668 & 137.809 \\
        & \Orkut & 686.753 & 14.543 & 41.391 & 62.687 & 78.799 & 93.299 & 109.459 & 125.168 & 138.031 & 142.816 & 153.518 \\
        & \USAfull & 1265.12 & 14.94 & 41.968 & 62.651 & 81.138 & 92.319 & 107.07 & 122.603 & 138.236 & 145.14 & 154.638 \\
        & \Lj & 1771.57 & 15.836 & 39.998 & 58.523 & 76.771 & 91.836 & 102.858 & 119.925 & 132.494 & 142.304 & 151.078 \\
        & \Pokec & 1836.48 & 13.713 & 33.944 & 51.317 & 65.858 & 79.525 & 91.648 & 105.713 & 119.703 & 125.42 & 133.795 \\
        & \Randtenm & 1997.8 & 12.49 & 33.543 & 50.217 & 65.146 & 81.143 & 91.7 & 109.491 & 118.233 & 129.908 & 132.396 \\
        & \BerkStan & 2038.24 & 14.521 & 41.089 & 60.521 & 79.346 & 91.101 & 105.424 & 119.842 & 134.504 & 146.716 & 152.602 \\
        & \Wikipedia & 412.304 & 16.478 & 40.385 & 61.875 & 79.863 & 90.295 & 107.666 & 123.892 & 136.74 & 147.073 & 155.606 \\
        & \Wikitalk & 1726.52 & 12.525 & 33.993 & 51.889 & 66.943 & 79.043 & 94.575 & 107.098 & 122.401 & 129.256 & 143.536 \\
        \hline
    \end{tabular}}
    \caption{Insertion benchmark (in millions of edges per second)}
    \label{tab:insertion-benchmark}
\end{table}


==> tables/graphquery.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{llrrrrrr}\hline
        \multirow{2}{*}{Data Structure} &  \multirow{2}{*}{Graph} &  \multicolumn{5}{c}{Batch Size } \\\cline{3-7}
        &   &  $2^{16}$ &  $2^{17}$ &  $2^{18}$ &  $2^{19}$ &  $2^{20}$ \\\hline
        \multirow{9}{*}{\textsc{Stinger (CPU)}} & \Higgs & 2.67 & 2.679 & 2.634 & 2.836 & 2.792 \\
        & \Orkut & 1.442 & 1.46 & 1.453 & 1.396 & 1.53 \\
        & \USAfull & 11.212 & 11.948 & 12.33 & 13.431 & 14.754 \\
        & \Lj & 3.495 & 3.467 & 3.64 & 3.646 & 4.399 \\
        & \Pokec & 3.849 & 3.907 & 4.003 & 3.701 & 4.595 \\
        & \Randtenm & 6.396 & 6.728 & 6.82 & 6.885 & 7.603 \\ 
        & \BerkStan & 5.969 & 6.365 & 6.361 & 5.756 & 7.489 \\
        & \Wikipedia & 2.042 & 2.05 & 2.018 & 2.079 & 2.123 \\
        & \Wikitalk & 0.186 & 0.179 & 0.182 & 0.183 & 0.184 \\
        \hline
        \multirow{9}{*}{\textsc{Hornet (GPU)}} & \Higgs & 363.197 & 460.121 & 544.449 & 593.001 & 630.287 \\
        & \Orkut & 166.168 & 147.81 & 253.6 & 297.106 & 404.623 \\
        & \USAfull & 909.628 & 877.846 & 844.955 & 828.11 & 823.546 \\
        & \Lj & 36.091 & 66.871 & 120.743 & 202.479 & 292.035 \\
        & \Pokec & 76.278 & 144.519 & 248.799 & 390.103 & 505.915 \\
        & \Randtenm & 464.623 & 382.035 & 414.238 & 482.454 & 537.175 \\
        & \BerkStan & 823.523 & 939.275 & 990.333 & 1035.38 & 1057.59 \\
        & \Wikipedia & 202.402 & 202.515 & 292.35 & 319.349 & 360.303 \\
        & \Wikitalk & 9.183 & 12.793 & 18.245 & 21.829 & 24.72 \\
        \hline
        \multirow{9}{*}{\textsc{\SG (GPU)}} & \Higgs & 897.655 & 1040.2 & 1065.45 & 1100.98 & 1129.71 \\
        & \Orkut & 861.454 & 964.914 & 1005.32 & 1029.46 & 1053.41 \\
        & \USAfull & 822.686 & 948.169 & 988.119 & 1017.71 & 1039.88 \\
        & \Lj & 870.401 & 949.632 & 989.641 & 1025.01 & 1049.13 \\
        & \Pokec & 841.597 & 940.954 & 987.252 & 1021.71 & 1046.77 \\
        & \Randtenm & 875.693 & 998.226 & 1039.65 & 1062.9 & 1091.6 \\
        & \BerkStan & 849.572 & 945.399 & 985.489 & 1014.18 & 1040 \\
        & \Wikipedia & 872.197 & 973.442 & 1012.21 & 1036.57 & 1059.79 \\
        & \Wikitalk & 1073.97 & 1260.36 & 1347.56 & 1408.68 & 1470.08 \\
        \hline
    \end{tabular}
    \caption{Query benchmark (in millions of edges per second)}\label{tab:query-benchmark}
\end{table}


==> tables/page-dec-large.tex <==
\begin{table}[h]
    \centering    
    \small
    \begin{tabular}{l >{\raggedleft\arraybackslash}p{1cm} >{\raggedleft\arraybackslash}p{1cm} >{\raggedleft\arraybackslash}p{1cm} >{\raggedleft\arraybackslash}p{1cm}}\hline
        \multirow{2}{*}{Graph} &  \multicolumn{4}{c}{Decremental Update Batch Size ($K = 10^3$)} \\\cline{2-5}
        &1K &10K &100K &1000K \\ \hline
        \Higgs & 36.982 & 36.947 & 44.99 & 80.423 \\
        \Orkut & 31.793 & 54.62 & 79.213 & 105.488 \\
        \USAfull & 113.373 & 299.366 & 565.065 & 817.422 \\
        \Lj & 25.772 & 49.55 & 86.521 & 151.757 \\
        \Pokec & 12.027 & 17.199 & 24.511 & 38.782 \\
        \Randtenm & 147.935 & 206.999 & 235.643 & 264.084 \\
        \BerkStan & 58.227 & 23.98 & 136.516 & 200.101 \\
        \Wikipedia & 28.038 & 54.742 & 93.661 & 158.321 \\
        \Wikitalk & 6.115 & 8.627 & 12.218 & 20.669 \\
    \hline
    \end{tabular}
    \caption{PageRank Decremental:  Performance of decremental batch updates performed on the full graph. Execution time in ms.}
    \label{tab:pagerank-dec-large}
\end{table}


==> tables/page-dec-small.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{llrrrrrrrrrr}\hline
        \multirow{2}{*}{Graph} & \multicolumn{10}{c}{Batch Update Average ($K = 10^3$)} \\\cline{2-11}
        & 1K & 2K & 3K & 4K & 5K & 6K & 7K & 8K & 9K & 10K \\ \hline
        \Higgs &20.861 &24.261 &28.906 &31.878 &34.405 &36.985 &34.839 &36.547 &36.949 &38.25 \\
        \Orkut &38.918 &52.985 &52.966 &54.715 &68.694 &70.453 &70.509 &70.488 &70.487 &70.45 \\
        \USAfull &130.455 &177.506 &223.682 &249.65 &270.658 &292.027 &293.938 &317.423 &335.754 &340.395 \\
        \Lj &38.125 &47.634 &57.142 &58.086 &64.752 &66.635 &66.626 &70.425 &76.136 &76.145 \\
        \Pokec &15.003 &17.963 &18.354 &20.348 &21.228 &20.938 &21.567 &22.111 &23.605 &23.958 \\
        \Randtenm &147.956 &177.555 &177.521 &177.495 &177.476 &207.041 &207.029 &207.043 &207.039 &207.037 \\
        \BerkStan &58.709 &69.666 &76.114 &83.621 &90.959 &96.035 &97.929 &101.921 &105.123 &108.092 \\
        \Wikipedia &36.539 &41.366 &49.917 &49.852 &52.326 &57.179 &60.835 &62.024 &68.145 &60.842 \\
        \Wikitalk &11.717 &13.034 &15.628 &16.777 &17.669 &19.643 &20.069 &20.986 &22.244 &23.17 \\
        \hline
    \end{tabular}
    \caption{PageRank Decremental: Performance of decremental batch updates in ms.}
    \label{tab:pagerank-dec-small}
\end{table}


==> tables/page-inc-large.tex <==
\begin{table}[h]
    \centering    
    \small
    \begin{tabular}{l >{\raggedleft\arraybackslash}p{1cm} >{\raggedleft\arraybackslash}p{1cm} >{\raggedleft\arraybackslash}p{1cm} >{\raggedleft\arraybackslash}p{1cm}}\hline
        \multirow{2}{*}{Graph} & \multicolumn{4}{c}{Incremental Update Batch Size ($K = 10^3$)} \\\cline{2-5}
        & 1K & 10K & 100K & 1000K \\
        \hline
        \Higgs &23.405 &23.881 &31.963 &53.774 \\
        \Orkut &18.266 &27.383 &54.972 &247.773 \\
        \USAfull &130.909 &319.349 &563.499 &821.524 \\
        \Lj &19.798 &31.039 &57.334 &163.489 \\
        \Pokec &8.352 &10.312 &16.257 &44.316 \\
        \Randtenm &81.897 &144.507 &174.258 &218.8 \\
        \BerkStan &50.006 &21.113 &139.804 &204.137 \\
        \Wikipedia &18.278 &33.649 &61.766 &164.635 \\
        \Wikitalk &6.195 &8.216 &12.296 &21.292 \\
    \hline
    \end{tabular}
    \caption{PageRank Incremental: Performance of incremental batch updates performed on 75\% of original graph. Execution time in ms.}
    \label{tab:pagerank-inc-large}
\end{table}


==> tables/page-inc-small.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{llrrrrrrrrrr}\hline
        \multirow{2}{*}{Graph}  & \multicolumn{10}{c}{Incremental Update Batch Size ($K = 10^3$)} \\\cline{2-11}
         & 1K  & 2K  & 3K  & 4K  & 5K  & 6K  & 7K  & 8K  & 9K  & 10K \\
        \hline 
        \Higgs  & 26.796  & 37.397  & 38.647  & 45.024  & 46.733  & 50.977  & 52.244  & 56.035  & 52.048  & 53.917 \\
        \Orkut  & 44.193  & 54.752  & 70.599  & 70.595  & 70.598  & 81.175  & 88.206  & 88.249  & 91.672  & 105.844 \\
        \USAfull  & 155.553  & 221.739  & 265.853  & 287.827  & 309.903  & 331.991  & 354.066  & 376.15  & 375.839  & 398.05 \\
        \Lj  & 47.673  & 57.211  & 66.707  & 66.725  & 76.272  & 76.258  & 84.838  & 85.802  & 85.766  & 88.677 \\
        \Pokec  & 15.174  & 17.972  & 18.571  & 21.167  & 21.266  & 20.961  & 21.781  & 22.764  & 23.656  & 24.028 \\
        \Randtenm  & 147.987  & 177.546  & 177.565  & 177.595  & 177.572  & 177.585  & 177.597  & 180.55  & 207.171  & 207.188 \\
        \BerkStan  & 90.085  & 109.125  & 117.163  & 126.692  & 128.704  & 134.84  & 138.195  & 138.304  & 138.5  & 141.283 \\
        \Wikipedia  & 38.973  & 49.916  & 56.041  & 62.041  & 65.817  & 69.342  & 74.233  & 90.104  & 84.011  & 85.14 \\
        \Wikitalk  & 11.644  & 13.935  & 14.344  & 15.801  & 16.135  & 16.852  & 17.017  & 17.53  & 17.614  & 17.821 \\
        \hline
    \end{tabular}
    \caption{PageRank Incremental: Performance of incremental batch updates in ms.}
    \label{tab:pagerank-inc-small}
\end{table}


==> tables/page-static.tex <==
\begin{table}[h]
  \centering
    \small
    \begin{tabular}{lrr} 
      \hline
      Graph & \textsc{Hornet} & \SG \\
      \hline
      \Higgs & 85.612 & 149.314 \\
      \Orkut & 744.344 & 551.652 \\
      \USAfull & 2366.233 & 1148.055 \\
      \Lj & 593.972 & 390.738 \\
      \Pokec & 236.329 & 94.984 \\
      \Randtenm & 966.913 & 325.427 \\
      \BerkStan & 103.039 & 256.255 \\
      \Wikipedia & 459.314 & 390.414 \\
      \Wikitalk & 113.047 & 61.782 \\
      \hline
  \end{tabular}
  \caption{PageRank - Static Running Time (ms)}
  \label{table:pagerank-static}
\end{table}

==> tables/sssp-decremental-large.tex <==
\begin{table}[h]
  \small
  \centering

  \begin{tabular}{lrrrr}
    \hline
    \multirow{2}{*}{Graph} & \multicolumn{4}{c}{Incremental Update Batch Size ($K = 10^3$)} \\\cline{2-5}
    & 1K & 10K & 100K & 1000K \\
    \hline
    \Higgs & 9.398 & 9.285 & 9.246 & 11.612 \\
    \Orkut & 32.183 & 32.434 & 32.984 & 39.716 \\
    \USAfull & 6842.068 & 5486.873 & 1695.826 & 6021.06 \\
    \Lj & 110.934 & 110.616 & 109.677 & 124.935 \\
    \Pokec & 45.854 & 45.637 & 45.09 & 57.697 \\
    \Randtenm & 234.467 & 249.22 & 247.01 & 319.881 \\
    \BerkStan & 21.542 & 21.381 & 15.192 & 13.819 \\
    \Wikipedia & 99.434 & 99.723 & 90.651 & 109.785 \\
    \Wikitalk & 27.334 & 32.938 & 29.189 & 38.612 \\
    \hline
  \end{tabular}
      
  \caption{SSSP Decremental: Performance of decremental batch updates performed on the full graph. Execution time in ms.}
  \label{table:sssp-decremental-large}
\end{table}

==> tables/sssp-decremental-small.tex <==
\begin{table}[h]
  \small
  \centering
  
  \begin{tabular}{lrrrrrrrrrr}
    \hline
    \multirow{2}{*}{Graph}  & \multicolumn{10}{c}{Incremental Update Batch Size ($K = 10^3$)} \\\cline{2-11}
    & 1K  & 2K  & 3K  & 4K  & 5K  & 6K  & 7K  & 8K  & 9K  & 10K \\
    \hline
    \Higgs & 8.911 & 9.455 & 9.622 & 9.546 & 9.451 & 9.601 & 9.564 & 9.551 & 9.602 & 9.69 \\
    \Orkut & 31.839 & 31.876 & 31.903 & 31.942 & 31.934 & 31.915 & 32.025 & 31.976 & 32.242 & 31.948 \\
    \USAfull & 973.11 & 1075.941 & 895.954 & 2261.207 & 720.452 & 724.939 & 814.415 & 871.867 & 1562.643 & 1194.677 \\
    \Lj & 90.381 & 95.203 & 100.014 & 105.036 & 108.628 & 100.083 & 109.569 & 101.617 & 102.911 & 105.48 \\
    \Pokec & 47.595 & 46.437 & 46.63 & 48.015 & 47.497 & 47.292 & 46.67 & 47.875 & 46.273 & 47.225 \\
    \Randtenm & 250.676 & 236.215 & 255.841 & 251.586 & 252.838 & 250.197 & 252.972 & 250.476 & 251.306 & 250.796 \\
    \BerkStan & 12.84 & 13.649 & 11.596 & 11.119 & 10.028 & 10.311 & 9.439 & 9.811 & 9.523 & 9.402 \\
    \Wikipedia & 98.077 & 90.8 & 97.904 & 99.489 & 100.679 & 93.687 & 92.63 & 99.705 & 100.221 & 98.871 \\
    \Wikitalk & 11.85 & 29.115 & 24.063 & 23.825 & 26.383 & 26.324 & 28.477 & 27.658 & 25.595 & 29.543 \\
    \hline
  \end{tabular}

  \caption{SSSP Decremental: Performance of decremental batch updates in ms.}
  \label{table:sssp-decremental-small}
\end{table}

==> tables/sssp-incremental-large.tex <==
\begin{table}[h]
  \small
  \centering

  \begin{tabular}{lrrrr}
    \hline
    \multirow{2}{*}{Graph} & \multicolumn{4}{c}{Incremental Update Batch Size ($K = 10^3$)} \\\cline{2-5}
    & 1K & 10K & 100K & 1000K \\
    \hline
    \Higgs & 0.66 & 0.81 & 3.735 & 9.905 \\
    \Orkut & 0.432 & 0.649 & 1.234 & 5.623 \\
    \USAfull & 2377.408 & 1258.736 & 577.633 & 236.146 \\
    \Lj & 0.905 & 1.116 & 8.31 & 57.743 \\
    \Pokec & 0.601 & 6.407 & 13.465 & 52.869 \\
    \Randtenm & 21.859 & 36.598 & 38.143 & 206.381 \\
    \BerkStan & 2.226 & 2.047 & 3.478 & 5.441 \\
    \Wikipedia & 7.621 & 20.646 & 17.791 & 75.692 \\
    \Wikitalk & 1.901 & 4.252 & 4.462 & 32.121 \\
    \hline
  \end{tabular}
      
  \caption{SSSP Incremental: Performance of incremental batch updates performed on 75\% of original graph. Execution time in ms.}
  \label{table:sssp-incremental-large}
\end{table}

==> tables/sssp-incremental-small.tex <==
\begin{table}[h]
  \small
  \centering

  \begin{tabular}{lrrrrrrrrrr}
    \hline
    \multirow{2}{*}{Graph}  & \multicolumn{10}{c}{Incremental Update Batch Size ($K = 10^3$)} \\\cline{2-11}
    & 1K  & 2K  & 3K  & 4K  & 5K  & 6K  & 7K  & 8K  & 9K  & 10K \\
    \hline
    \Higgs & 3.355 & 2.564 & 3.44 & 2.912 & 3.035 & 3.086 & 3.063 & 2.956 & 2.836 & 2.766 \\
    \Orkut & 0.231 & 0.258 & 0.268 & 0.306 & 0.319 & 0.329 & 0.362 & 0.348 & 0.3 & 0.355 \\
    \USAfull & 788.675 & 594.821 & 629.125 & 561.426 & 499.753 & 577.348 & 517.357 & 460.203 & 471.188 & 421.911 \\
    \Lj & 13.002 & 14.614 & 21.718 & 14.097 & 17.623 & 15.009 & 20.46 & 20.191 & 16.497 & 21.553 \\
    \Pokec & 16.506 & 11.889 & 12.018 & 12.124 & 15.309 & 13.659 & 11.291 & 14.291 & 11.824 & 11.752 \\
    \Randtenm & 11.517 & 28.354 & 36.23 & 34.396 & 30.757 & 26.007 & 39.922 & 39.485 & 39.839 & 41.473 \\
    \BerkStan & 11.759 & 9.216 & 6.849 & 6.298 & 5.44 & 4.666 & 4.608 & 3.793 & 4.102 & 3.806 \\
    \Wikipedia & 21.641 & 23.374 & 23.321 & 30.764 & 28.47 & 19.486 & 24.793 & 16.985 & 25.022 & 19.31 \\
    \Wikitalk & 2.666 & 3.393 & 6.389 & 2.97 & 5.378 & 8.965 & 7.729 & 9.195 & 7.095 & 4.977 \\
    \hline
  \end{tabular}

  \caption{SSSP Incremental: Performance of incremental batch updates in ms.}
  \label{table:sssp-incremental-small}
\end{table}

==> tables/sssp-static.tex <==
\begin{table}[h]
  \small
  \centering

  \begin{tabular}{lrrrr}\hline
    Graph & Hornet & \name & \name (tree) \\
    \hline
    \Higgs & 15.031 & 13.13 & 17.098 \\
    \Orkut & 607.53 & 518.82 & 656.412 \\
    \USAfull & 8798.186 & 1666.77 & 5843.45 \\
    \Lj & 262.741 & 153.84 & 210.871 \\
    \Pokec & 89.961 & 78.37 & 105.725 \\
    \Randtenm & 602.086 & 328.76 & 333.826 \\
    \BerkStan & 37.755 & 15.86 & 24.508 \\
    \Wikipedia & 132.661 & 127.59 & 168.553 \\
    \Wikitalk & 11.366 & (todo) & 37.465 \\
    \hline
    \end{tabular}
    
  \caption{SSSP Static: Hornet vs. \name. Execution time in ms.}
  \label{table:sssp-static}
\end{table}

==> tables/tc-dec-large.tex <==
\begin{table}[h]
    \centering    
    \small
    \begin{tabular}{l >{\raggedleft\arraybackslash}p{1cm} >{\raggedleft\arraybackslash}p{1cm} >{\raggedleft\arraybackslash}p{1cm} >{\raggedleft\arraybackslash}p{1cm}}\hline
        \multirow{2}{*}{Graph} &  \multicolumn{4}{c}{Decremental Update Batch Size ($K = 10^3$)} \\\cline{2-5}
        &  1K &  10K &  100K &  1000K \\\hline 
        \Higgs & 7.562 & 12.546 & 48.981 & 226.908 \\
        \Orkut & 3.535 & 8.972 & 22.741 & 101.608 \\
        \USAfull & 0.221 & 0.219 & 0.51 & 3.27 \\
        \Lj & 1.843 & 4.288 & 10.764 & 45.057 \\
        \Pokec & 1.75 & 3.049 & 7.764 & 36.394 \\
        \BerkStan & 0.804 & 17.235 & 43.483 & 207.245 \\
        \Wikipedia & 4.253 & 10.298 & 59.25 & 272.172 \\
        \Wikitalk & 3.019 & 18.559 & 72.572 & 421.549 \\
    \hline
    \end{tabular}
    \caption{Triangle Counting: Performance of decremental batch updates performed on the full graph. Execution time in ms.}
    \label{tab:tc-dec-large}
\end{table}


==> tables/tc-inc-large.tex <==
\begin{table}[h]
    \centering    
    \small
    \begin{tabular}{l >{\raggedleft\arraybackslash}p{1cm} >{\raggedleft\arraybackslash}p{1cm} >{\raggedleft\arraybackslash}p{1cm} >{\raggedleft\arraybackslash}p{1cm}}\hline
        \multirow{2}{*}{Graph} &  \multicolumn{4}{c}{Incremental Update Batch Size ($K = 10^3$)} \\\cline{2-5}
        &  1K &  10K &  100K &  1000K \\\hline 
        \Higgs & 7.056 & 12.579 & 55.767 & 238.144 \\
        \Orkut & 3.534 & 8.619 & 23.48 & 110.067 \\
        \USAfull & 0.235 & 0.224 & 0.534 & 3.516 \\
        \Lj & 1.98 & 4.495 & 10.398 & 48.274 \\
        \Pokec & 1.678 & 2.779 & 7.524 & 37.579 \\
        \BerkStan & 1.167 & 17.18 & 44.249 & 205.674 \\
        \Wikipedia & 4.169 & 10.467 & 55.858 & 277.662 \\
        \Wikitalk & 3.298 & 18.44 & 69.428 & 404.52 \\
    \hline
    \end{tabular}
    \caption{Triangle Counting: Performance of incremental batch updates performed on 75\% of the original graph. Execution time in ms.}
    \label{tab:tc-inc-large}
\end{table}


==> tables/tc_dec.tex <==
\begin{table}[h]
    \small
    \centering
    \begin{tabular}{lrrrrrrrrrrr}\hline
      \multirow{2}{*}{Graph} &   \multicolumn{10}{c}{Decremental Update Batch Size (K = $10^3$)} \\\cline{2-11}
      &   1K &   2K &   3K &   4K &   5K &   6K &   7K &    8K &   9K &   10K \\
      \hline
      \Higgs & 1.367 & 1.429 & 1.988 & 1.995 & 2.673 & 2.673 & 2.727 & 2.445 & 2.384 & 2.601 \\
      \Orkut & 2.094 & 2.521 & 2.637 & 2.972 & 3.072 & 3.072 & 3.212 & 3.1 & 3.408 & 3.347 \\
      \USAfull & 0.12 & 0.121 & 0.129 & 0.141 & 0.184 & 0.184 & 0.19 & 0.159 & 0.163 & 0.166 \\
      \Lj & 0.729 & 0.896 & 0.819 & 0.988 & 0.977 & 0.977 & 1.045 & 1.116 & 1.159 & 1.158 \\
      \Pokec & 0.702 & 0.752 & 0.793 & 0.828 & 0.848 & 0.848 & 0.874 & 0.998 & 0.959 & 1.004 \\
      \BerkStan & 0.503 & 0.526 & 0.608 & 0.599 & 0.971 & 0.971 & 1.02 & 0.725 & 0.847 & 1.117 \\
      \Wikipedia & 1.862 & 1.631 & 1.822 & 1.951 & 2.363 & 2.363 & 2.199 & 2.501 & 2.823 & 2.694 \\
      \Wikitalk & 0.241 & 0.844 & 0.781 & 0.606 & 0.956 & 0.956 & 1.308 & 1.141 & 1.162 & 1.388 \\
      \hline
    \end{tabular}
    \caption{Triange Counting: Performance of decremental batch updates in ms.}
    \label{table:triangle-counting-decremental-small}
\end{table}


==> tables/tc_inc.tex <==
\begin{table}[h]
    \small
    \centering
    \begin{tabular}{lrrrrrrrrrrr}\hline
      \multirow{2}{*}{Graph} &  \multicolumn{10}{c}{Incremetal Update Batch Size (K = $10^3$)} \\\cline{2-11}
      &  1K &  2K &  3K &  4K &  5K &  6K &  7K &   8K &  9K &  10K \\
      \hline
      \Higgs & 0.708 & 0.761 & 0.885 & 0.988 & 0.975 & 0.975 & 1.319 & 1.077 & 1.157 & 1.462 \\
      \Orkut & 1.141 & 1.186 & 1.26 & 1.492 & 1.443 & 1.443 & 1.498 & 1.465 & 1.725 & 1.546 \\
      \USAfull & 0.146 & 0.136 & 0.146 & 0.159 & 0.17 & 0.17 & 0.172 & 0.174 & 0.178 & 0.182 \\
      \Lj & 0.328 & 0.311 & 0.351 & 0.376 & 0.402 & 0.402 & 0.407 & 0.43 & 0.471 & 0.478 \\
      \Pokec & 0.428 & 0.45 & 0.493 & 0.498 & 0.537 & 0.537 & 0.568 & 0.583 & 0.575 & 0.624 \\
      \BerkStan & 0.279 & 0.276 & 0.352 & 0.359 & 0.388 & 0.388 & 0.371 & 0.4 & 0.365 & 0.44 \\
      \Wikipedia & 0.47 & 0.584 & 0.718 & 0.777 & 0.75 & 0.75 & 0.806 & 0.797 & 0.797 & 0.854 \\
      \Wikitalk & 0.116 & 0.124 & 0.131 & 0.164 & 0.161 & 0.161 & 0.167 & 0.214 & 0.202 & 0.18 \\
      \hline
    \end{tabular}
    \caption{Triange Counting: Performance of incremental batch updates in ms.}
    \label{table:triangle-counting-incremental-small}
\end{table}


==> tables/tc_static.tex <==
\begin{table}[h]
  \centering
  \begin{tabular}{lrr}
    \hline
    Graph &  Average (ms) \\
    \hline
    \Higgs & 1576.593 \\
    \Orkut & 23466.98 \\
    \USAfull & 54.797 \\
    \Lj & 3194.504 \\
    \Pokec & 1566.077 \\
    \BerkStan & 280.939 \\
    \Wikipedia & 12760.41 \\
    \Wikitalk & 497.927 \\
    \hline
  \end{tabular}
  \caption{Triangle Counting - Static Running Time (ms)}
  \label{table:triangle-counting-static}
\end{table}


==> tables/wcc-partial-75.tex <==
\begin{table}
    \small
      \centering
        \begin{tabular}{p{0.1\textwidth} l r r r r r}
          \hline
          \multirow{2}{0.1\textwidth}{Method}                                                          & \multirow{2}{0.07\textwidth}{Dataset} & \multicolumn{4}{c}{Update Batch Size (K = $10^3$ )}                                          \\ \cline{3-6}
                                                                                                        &                                       & 1K                                  & 10K  & 100K  & 1000K \\      \hline
     
    \multirow{9}{0.1\textwidth}{SlabIterator} & \Higgs & 13.2$\times$ & 5.52$\times$ & 2.11$\times$ & 1.22$\times$ \\
     & \Lj & 20.84$\times$ & 10.07$\times$ & 7.28$\times$ & 2.83$\times$ \\
     & \Pokec & 9.17$\times$ & 6.77$\times$ & 5.41$\times$ & 1.9$\times$ \\
     & \Randtenm & 129.9$\times$ & 120.8$\times$ & 83.0$\times$ & 16.7$\times$ \\
     & \BerkStan & 11.94$\times$ & 5.89$\times$ & 2.26$\times$ & 1.17$\times$ \\
     & \Wikitalk & 1.24$\times$ & 1.19$\times$ & 1.19$\times$ & 1.16$\times$ \\
     & \Wikipedia & 28.09$\times$ & 19.5$\times$ & 6.07$\times$ & 3.6$\times$ \\
     & \Orkut & 74.6$\times$ & 25.9$\times$ & 19.3$\times$ & 4.45$\times$ \\
     & \USAfull & 25.5$\times$ & 25.0$\times$ & 21.2$\times$ & 10.3$\times$ \\
    \hline
    \multirow{9}{0.1\textwidth}{UpdateIterator} & \Higgs & 22.8$\times$ & 6.24$\times$ & 1.64$\times$ & 0.92$\times$ \\
     & \Lj & 42.8$\times$ & 11.7$\times$ & 5.57$\times$ & 2.31$\times$ \\
     & \Pokec & 43.0$\times$ & 9.23$\times$ & 4.26$\times$ & 1.43$\times$ \\
     & \Randtenm & 136.9$\times$ & 132.2$\times$ & 80.9$\times$ & 15.7$\times$ \\
     & \BerkStan & 14.1$\times$ & 6.0$\times$ & 1.8$\times$ & .89$\times$ \\
     & \Wikitalk & 8.94$\times$ & 1.76$\times$ & .99$\times$ & 1.0$\times$ \\ 
     & \Wikipedia & 51.8$\times$ & 20.2$\times$ & 5.01$\times$ & 3.02$\times$ \\
     & \Orkut & 120.2$\times$ & 28.8$\times$ & 15.6$\times$ & 3.62$\times$ \\
     & \USAfull & 25.4$\times$ & 24.8$\times$ & 20.8$\times$ & 8.48$\times$ \\
    \hline
    \multirow{9}{0.1\textwidth}{UpdateIterator + Single Bucket} & \Higgs & 25.1$\times$ & 8.67$\times$ & 2.4$\times$ & 1.22$\times$ \\
     & \Lj & 50.27$\times$ & 17.4$\times$ & 8.43$\times$ & 2.83$\times$ \\
     & \Pokec & 48.6$\times$ & 13.3$\times$ & 6.34$\times$ & 1.81$\times$ \\
     & \Randtenm & 136.7$\times$ & 132.4$\times$ & 79.8$\times$ & 16.1$\times$ \\
     & \BerkStan & 15.41$\times$ & 7.9$\times$ & 2.8$\times$ & 1.12$\times$ \\
     & \Wikitalk & 23.3$\times$ & 3.19$\times$ & 2.04$\times$ & 1.93$\times$ \\
     & \Wikipedia & 75.8$\times$ & 35.7$\times$ & 7.98$\times$ & 4.04$\times$ \\
     & \Orkut & 187.5$\times$ & 49.7$\times$ & 24.8$\times$ & 5.38$\times$ \\
     & \USAfull & 25.4$\times$ & 24.8$\times$ & 21.2$\times$ & 8.95$\times$ \\
    \hline
        \end{tabular}
        \caption{WCC: Performance of batch updates over 75\% edges sampled from the original graph vs. the na\"{i}ve scheme}
      \label{table:partial75}
    \end{table}

==> tables/wcc-static.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{lrrr}
    \hline
    Graph &\textsc{Stinger} ($\times 10^3$) &\textsc{Hornet} &\textsc{\SG} \\
    \hline
    \Higgs &0.255 &2.804 &1.105 \\
    \Orkut &- &23.223 &24.562 \\
    \USAfull &128.077 &693.477 &29.729 \\
    \Lj &2.181 &19.741 &11.596 \\
    \Pokec &0.594 &7.489 &3.721 \\
    \Randtenm &4.324 &69.256 &37.368 \\
    \BerkStan &1.416 &21.185 &1.051 \\
    \Wikipedia &2.78 &14.935 &9.681 \\
    \Wikitalk &0.439 &3.252 &4.935 \\
    \hline
    \end{tabular}
    \caption{Performance of Static Weakly-Connected Components (in milliseconds)}
    \label{tab:static-wcc}
\end{table}
